Illuminating the Unseen: Investigating the Context-induced Harms in Behavioral Sensing

Behavioral sensing technologies are rapidly evolving across a range of well-being applications. Despite its potential, concerns about the responsible use of such technology are escalating. In response, recent research within the sensing technology has started to address these issues. While promising, they primarily focus on broad demographic categories and overlook more nuanced, context-specific identities. These approaches lack grounding within domain-specific harms that arise from deploying sensing technology in diverse social, environmental, and technological settings. Additionally, existing frameworks for evaluating harms are designed for a generic ML life cycle, and fail to adapt to the dynamic and longitudinal considerations for behavioral sensing technology. To address these gaps, we introduce a framework specifically designed for evaluating behavioral sensing technologies. This framework emphasizes a comprehensive understanding of context, particularly the situated identities of users and the deployment settings of the sensing technology. It also highlights the necessity for iterative harm mitigation and continuous maintenance to adapt to the evolving nature of technology and its use. We demonstrate the feasibility and generalizability of our framework through post-hoc evaluations on two real-world behavioral sensing studies conducted in different international contexts, involving varied population demographics and machine learning tasks. Our evaluations provide empirical evidence of both situated identity-based harm and more domain-specific harms, and discuss the trade-offs introduced by implementing bias mitigation techniques.

==> fig_tab_alg/demographics.tex <==
\begin{table}[htb!]
    \centering
    \small
    \caption{\textbf{Demographics of Sensitive Attributes.}}
   \renewcommand{\arraystretch}{1}
   \resizebox{0.65\textwidth}{!}{
\begin{tabular}[t]{l|l|rrrr}
\hline \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell[c]{Sensitive\\ Attributes}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\makecell[c]{(Un)protected \\ Groups}}}} & \multicolumn{4}{c}{\textbf{Number (\%)}} \\\cline{3-6} %& \multicolumn{4}{c}{\textbf{(Min, Max)}}\\\cline{3-18}
         & & \makecell[c]{\textbf{DS1}} & \makecell[c]{\textbf{DS2}} & \makecell[c]{\textbf{DS3}} & \makecell[c]{\textbf{DS4}} \\\hline
         \multirow{2}{*}{Gender} & Non-male & 95 (68\%) & 102 (50\%) & 71 (55\%) &  121 (65\%) \\   
         & Male & 44 (32\%) & 101 (50\%) & 59 (45\%) & 64 (35\%) \\\hline
         \multirow{3}{*}{Race} & Asian & 67 (48\%) & 97 (48\%) & 72 (55\%) & 99 (54\%)  \\
         % & Non-Asian & 72 (52\%) &  &  &  & 
         %  &  &  &  \\
         & Biracial & 
         19 (14\%) & 22 (11\%) & 9 (7\%) & 18 (10\%)  \\
          % & Non-Biracial & 120 (86\%) &  &  &  & 
          % &  &  &  \\
         & White & 
         44 (32\%) & 68 (34\%) & 39 (30\%) & 48 (26\%) \\\hline
          % & Non-White & &  &  &  & 
          % &  &  &  \\\hline
        \multirow{2}{*}{\makecell[l]{First-gen \\ College Student}} & First-gen & 
        44 (32\%) & 62 (31\%) & 45 (35\%) & 67 (36\%) \\
         & Non-first-gen & 
         95 (68\%) & 141 (69\%) & 85 (65\%) & 118 (64\%) \\\hline
         \multirow{2}{*}{\makecell[l]{Sexual \\Orientation}} & Non-heterosexual & 
         17 (12\%) & 15 (7\%) & 22 (17\%) & 39 (21\%) \\ 
         & Heterosexual & 
         122 (88\%) & 188 (93\%) & 108 (83\%) & 146 (79\%) \\\hline
         \multirow{2}{*}{\makecell[l]{Mother's \\ Education}} & Below Bachelor & 
         56 (40\%) & 81 (40\%) & 57 (44\%) & 72 (39\%) \\
         & Bachelor or Higher & 
         83 (60\%) & 122 (60\%) & 73 (56\%) & 113 (61\%) \\\hline
         \multirow{2}{*}{\makecell[l]{Father's \\ Education}} & Below Bachelor & 
         55 (40\%) & 78 (38\%) & 59 (45\%) & 85 (46\%) \\
         & Bachelor or Higher & 
         84 (60\%) & 125 (62\%) & 71 (55\%) & 100 (54\%) \\\hline
         \multirow{2}{*}{\makecell[l]{Immigration \\ Status}} & Immigrant & 
         31 (22\%) & 52 (26\%) & 33 (25\%) & 43 (23\%) \\
         & Non-immigrant & 
         108 (78\%) & 151 (74\%) & 97 (75\%) & 142 (77\%) \\\hline
       
    \end{tabular}}
    \label{tab:demo}
\end{table}

==> fig_tab_alg/fig_case_study2_emotional_TP.tex <==
\begin{figure}[t]
    \centering
    \caption{\textbf{Comparative Overview of Data Distributions Across Various Groups}. The upper figure highlights the disparity in emotional engagement prediction errors (Ground Truth - Prediction) between students comfortable with the current temperature (more scattered) versus those preferring warmer or cooler settings (more centralized). The lower figure delineates the difference in prediction errors for students in room 41 (predominantly above the dashed line) as compared to those in other language rooms (more evenly distributed). }
    \subfloat[Temperature Comfort, Emotional Engagement]{\includegraphics[scale=0.45]{figures/emotional_TP.png}
    \label{fig:emotional_TP}}

    \subfloat[Language Room, Emotional Engagement]{\includegraphics[scale=0.337]{figures/emotional_Language_Room.png}
    \label{fig:emotional_language_room}}

    
\end{figure}


==> fig_tab_alg/reproduction_results.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.36]{figures/reproduction_results.png}
    \caption{reproduction results. DS1 and DS2 were used in prior work \cite{xu2023globem} and DS3 and DS4 are newly reported in this study. Performance comparison of the algorithms on DS1 and DS2 allows for reproduction analysis, while evaluation on DS3 and DS4 provides additional insights into the algorithmic fairness. $\Delta$ represents the difference between our results and prior reported results. \han{need to reframe}}
    \label{fig:reproduction_results}
\end{figure}

==> fig_tab_alg/tab_acc_w_t_demo.tex <==
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\caption{Algorithmic fairness evaluation results through the \textbf{disparity in accuracy} (without incorporating demographic data into the training and testing process). The p-value serves as a significance threshold, indicating the likelihood that the observed data could have occurred by random chance before applying the Benjamini-Hochberg correction, while the q-value is the adjusted p-value by Benjamini-Hochberg correction. Significance is marked *$<0.05$, **$<0.01$, ***$<0.001$. Our analyses and conclusions are based on q-values.}
\resizebox{0.9\textwidth}{!}{\begin{tabular}{|l|l|rr|rr|rr|rr|}\hline
&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\\cline{3-10}
\multirow{-2}{*}{\textbf{Algorithms}} &\multirow{-2}{*}{\textbf{Sensitive Attributes}} & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  \\\hline

  \multirow{5}{*}{Wahle \etal \cite{wahle2016mobile}} & First-gen College Student & \cellcolor[HTML]{F4CCCC}*0.034 & 0.020 & \cellcolor[HTML]{E06666}***0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.507 & 0.020 & \cellcolor[HTML]{F4CCCC}*0.013 & 0.010 \\
  & Gender & 0.063 & 0.030 & \cellcolor[HTML]{EA9999}**0.004 & \cellcolor[HTML]{F4CCCC}*0.020 & 0.785 & 0.050 & 0.718 & 0.050 \\
  & Immigration Status & 0.087 & 0.040 & 0.852 & 0.040 & 0.426 & 0.010 & 0.628 & 0.040 \\
  & Race & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.433 & 0.030 & 0.609 & 0.030 & 0.114 & 0.020 \\
  & Sexual Orientation & 0.255 & 0.050 & 0.858 & 0.050 & 0.684 & 0.040 & 0.537 & 0.030 \\
\hline

\multirow{5}{*}{Saeb \etal \cite{saeb2015mobile}} & First-gen College Student & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & \cellcolor[HTML]{EA9999}**0.002 & \cellcolor[HTML]{F4CCCC}*0.020 & 0.079 & 0.010 & \cellcolor[HTML]{EA9999}**0.007 & \cellcolor[HTML]{F4CCCC}*0.020 \\
  & Gender & 0.305 & 0.050 & \cellcolor[HTML]{EA9999}**0.005 & \cellcolor[HTML]{F4CCCC}*0.030 & 0.247 & 0.020 & 0.083 & 0.040 \\
  & Immigration Status & \cellcolor[HTML]{E06666}***0.001 & \cellcolor[HTML]{F4CCCC}*0.020 & \cellcolor[HTML]{EA9999}**0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.507 & 0.040 & 0.362 & 0.050 \\
  & Race & \cellcolor[HTML]{EA9999}**0.001 & \cellcolor[HTML]{F4CCCC}*0.030 & \cellcolor[HTML]{EA9999}**0.009 & \cellcolor[HTML]{F4CCCC}*0.040 & 0.892 & 0.050 & 0.075 & 0.030 \\
  & Sexual Orientation & 0.138 & 0.040 & 0.292 & 0.050 & 0.406 & 0.030 & \cellcolor[HTML]{EA9999}**0.003 & \cellcolor[HTML]{F4CCCC}*0.010 \\
\hline

\multirow{5}{*}{Farhan \etal \cite{farhan2016behavior}} & First-gen College Student & 0.401 & 0.030 & 0.152 & 0.020 & 0.736 & 0.030 & 0.278 & 0.030 \\
  & Gender & 0.377 & 0.020 & \cellcolor[HTML]{EA9999}**0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.776 & 0.040 & \cellcolor[HTML]{F4CCCC}*0.019 & 0.010 \\
  & Immigration Status & 0.566 & 0.040 & 0.237 & 0.040 & 0.868 & 0.050 & 0.459 & 0.050 \\
  & Race & 0.681 & 0.050 & 0.976 & 0.050 & \cellcolor[HTML]{F4CCCC}*0.020 & 0.010 & 0.415 & 0.040 \\
  & Sexual Orientation & 0.158 & 0.010 & 0.222 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.042 & 0.020 & 0.134 & 0.020 \\
\hline

\multirow{5}{*}{Canzian \etal \cite{canzian2015trajectories}} & First-gen College Student & \cellcolor[HTML]{F4CCCC}*0.034 & 0.020 & \cellcolor[HTML]{EA9999}**0.008 & \cellcolor[HTML]{F4CCCC}*0.020 & 0.107 & 0.020 & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 \\
  & Gender & 0.063 & 0.030 & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.360 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.039 & 0.030 \\
  & Immigration Status & 0.087 & 0.040 & \cellcolor[HTML]{F4CCCC}*0.014 & \cellcolor[HTML]{F4CCCC}*0.030 & 0.469 & 0.050 & 0.489 & 0.050 \\
  & Race & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.433 & 0.050 & 0.086 & 0.010 & 0.081 & 0.040 \\
  & Sexual Orientation & 0.255 & 0.050 & 0.188 & 0.040 & 0.374 & 0.040 & \cellcolor[HTML]{EA9999}**0.006 & \cellcolor[HTML]{F4CCCC}*0.020 \\
\hline
 
\multirow{5}{*}{Wang \etal \cite{wang2018tracking}} & First-gen College Student & \cellcolor[HTML]{F4CCCC}*0.033 & 0.020 & \cellcolor[HTML]{EA9999}**0.002 & \cellcolor[HTML]{F4CCCC}*0.020 & 0.183 & 0.040 & \cellcolor[HTML]{EA9999}**0.007 & \cellcolor[HTML]{F4CCCC}*0.020 \\
  & Gender & 0.277 & 0.040 & \cellcolor[HTML]{EA9999}**0.003 & \cellcolor[HTML]{F4CCCC}*0.030 & 0.358 & 0.050 & 0.093 & 0.040 \\
  & Immigration Status & \cellcolor[HTML]{EA9999}**0.006 & \cellcolor[HTML]{F4CCCC}*0.010 & \cellcolor[HTML]{EA9999}**0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & \cellcolor[HTML]{F4CCCC}*0.026 & 0.010 & 0.889 & 0.050 \\
  & Race & 0.202 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.012 & \cellcolor[HTML]{F4CCCC}*0.040 & 0.063 & 0.020 & 0.060 & 0.030 \\
  & Sexual Orientation & 0.309 & 0.050 & 0.307 & 0.050 & 0.064 & 0.030 & \cellcolor[HTML]{E06666}***0.001 & \cellcolor[HTML]{F4CCCC}*0.010 \\
\hline

\multirow{5}{*}{Lu \etal \cite{lu2018joint}} & First-gen College Student & \cellcolor[HTML]{EA9999}**0.003 & \cellcolor[HTML]{F4CCCC}*0.010 & \cellcolor[HTML]{F4CCCC}*0.021 & 0.010 & 0.499 & 0.040 & 0.964 & 0.050 \\
& Gender & 0.955 & 0.050 & 0.409 & 0.040 & 0.484 & 0.030 & 0.064 & 0.020 \\
& Immigration Status & 0.719 & 0.040 & 0.534 & 0.050 & 0.745 & 0.050 & \cellcolor[HTML]{F4CCCC}*0.049 & 0.010 \\
& Race & 0.072 & 0.020 & 0.150 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.035 & 0.010 & 0.573 & 0.040 \\
& Sexual Orientation & 0.707 & 0.030 & 0.097 & 0.020 & \cellcolor[HTML]{F4CCCC}*0.036 & 0.020 & 0.106 & 0.030 \\
\hline
 
 \multirow{5}{*}{Xu\_interpretable \etal \cite{xu2019leveraging}} & First-gen College Student & 0.239 & 0.040 & 0.180 & 0.010 & 0.211 & 0.010 & 0.447 & 0.030 \\
  & Gender & 0.172 & 0.020 & 0.256 & 0.020 & 0.607 & 0.040 & 0.216 & 0.010 \\
  & Immigration Status & 0.219 & 0.030 & 0.642 & 0.050 & 0.506 & 0.030 & 0.978 & 0.050 \\
  & Race & 0.151 & 0.010 & 0.256 & 0.030 & 0.275 & 0.020 & 0.542 & 0.040 \\
  & Sexual Orientation & 0.330 & 0.050 & 0.556 & 0.040 & 0.838 & 0.050 & 0.392 & 0.020 \\
\hline
 
 \multirow{5}{*}{Xu\_personalized \etal \cite{xu2021leveraging}} & First-gen College Student & 0.548 & 0.030 & 0.058 & 0.030 & 0.696 & 0.030 & 0.294 & 0.020 \\
  & Gender & 0.355 & 0.010 & 0.313 & 0.040 & 0.910 & 0.050 & 0.842 & 0.050 \\
  & Immigration Status & 0.742 & 0.050 & \cellcolor[HTML]{F4CCCC}*0.023 & 0.020 & 0.185 & 0.010 & 0.629 & 0.040 \\
  & Race & 0.428 & 0.020 & \cellcolor[HTML]{E06666}***0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.396 & 0.020 & 0.343 & 0.030 \\
  & Sexual Orientation & 0.658 & 0.040 & 0.731 & 0.050 & 0.825 & 0.040 & 0.066 & 0.010 \\
\hline
 
%  \multirow{5}{*}{Chikersal \etal \cite{chikersal2021detecting}} & First-gen College Student & 0.826 & 0.030 & 0.238 & 0.020 & 0.107 & 0.010 & \cellcolor[HTML]{F4CCCC}*0.027 & 0.010 \\
%   & Gender & 0.992 & 0.050 & 0.916 & 0.040 & 0.472 & 0.030 & 0.582 & 0.040 \\
%   & Immigration Status & 0.946 & 0.040 & 0.073 & 0.010 & 0.812 & 0.050 & 0.879 & 0.050 \\
%   & Race & 0.654 & 0.020 & 0.921 & 0.050 & 0.279 & 0.020 & 0.090 & 0.020 \\
%   & Sexual Orientation & \cellcolor[HTML]{F4CCCC}*0.027 & 0.010 & 0.416 & 0.030 & 0.660 & 0.040 & 0.129 & 0.030 \\
% \hline
 
\end{tabular}}
\label{tab_acc_w_t_demo}
\end{table}

==> fig_tab_alg/tab_all_w_t_demo_simplified.tex <==
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\caption{Algorithmic fairness evaluation results through the disparity in accuracy, the disparity in false negative rate, and the disparity in false positive rate (without incorporating demographic data into the training and testing process). The results are adjusted p-values by Benjamini-Hochberg correction after the Mann-Whitney U test. Significance is highlighted in red. Acc, Fnr, and Fpr are the abbreviations of the disparity in accuracy, the disparity in false negative rate, and the disparity in false positive rate.}
\resizebox{0.95\textwidth}{!}{\begin{tabular}{|l|l|ccc|ccc|ccc|ccc|}\hline
&&
\multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\\cline{3-14}
\multirow{-2}{*}{\textbf{Algorithms}} &\multirow{-2}{*}{\textbf{Sensitive Attributes}} & \multicolumn{1}{c}{Acc}  & \multicolumn{1}{c}{Fnr}  & \multicolumn{1}{c|}{Fpr}  & \multicolumn{1}{c}{Acc}  & \multicolumn{1}{c}{Fnr}  & \multicolumn{1}{c|}{Fpr}  & \multicolumn{1}{c}{Acc}  & \multicolumn{1}{c}{Fnr}  & \multicolumn{1}{c|}{Fpr}  & \multicolumn{1}{c}{Acc}  & \multicolumn{1}{c}{Fnr}  & \multicolumn{1}{c|}{Fpr}  \\\hline

  \multirow{5}{*}{Wahle \etal \cite{wahle2016mobile}} & First-gen College Student & & & &  \cellcolor[HTML]{F4CCCC}Y & & \cellcolor[HTML]{F4CCCC}Y & & & & & & \\
  & Gender & & & & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & \\
  & Immigration Status & & & & & & & & & & & & \\
  & Race & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & & & & \\
  & Sexual Orientation & & & & & & & & & & & & \\
\hline

\multirow{5}{*}{Saeb \etal \cite{saeb2015mobile}} & First-gen College Student & \cellcolor[HTML]{F4CCCC}Y & & & \cellcolor[HTML]{F4CCCC}Y & & & & & & \cellcolor[HTML]{F4CCCC}Y & &\\
  & Gender & & & & \cellcolor[HTML]{F4CCCC}Y & & & & & \cellcolor[HTML]{F4CCCC}Y &  & & \\
  & Immigration Status & \cellcolor[HTML]{F4CCCC}Y &\cellcolor[HTML]{F4CCCC}Y & &  \cellcolor[HTML]{F4CCCC}Y & & & & & & & &\\
  & Race & \cellcolor[HTML]{F4CCCC}Y & & & \cellcolor[HTML]{F4CCCC}Y & & & & & \cellcolor[HTML]{F4CCCC}Y &  & &\\
  & Sexual Orientation & & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & \cellcolor[HTML]{F4CCCC}Y & \cellcolor[HTML]{F4CCCC}Y & \\
\hline

\multirow{5}{*}{Farhan \etal \cite{farhan2016behavior}} & First-gen College Student & & & & & & & & & & & & \\
  & Gender & & & &  \cellcolor[HTML]{F4CCCC}Y & & & & & & & & \\
  & Immigration Status & & & & & \cellcolor[HTML]{F4CCCC}Y & & & & & & & \\
  & Race & & & & & & & & & \cellcolor[HTML]{F4CCCC}Y & & &\\
  & Sexual Orientation & & & & & & & & & \cellcolor[HTML]{F4CCCC}Y & & & \\
\hline

\multirow{5}{*}{Canzian \etal \cite{canzian2015trajectories}} & First-gen College Student & & & & \cellcolor[HTML]{F4CCCC}Y & & \cellcolor[HTML]{F4CCCC}Y & & & & \cellcolor[HTML]{F4CCCC}Y & & \\
  & Gender & & & & \cellcolor[HTML]{F4CCCC}Y & & \cellcolor[HTML]{F4CCCC}Y & & & &  & & \\
  & Immigration Status & & & & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & \\
  & Race & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & \cellcolor[HTML]{F4CCCC}Y & & & \\
  & Sexual Orientation & & & & & & & & & & \cellcolor[HTML]{F4CCCC}Y & & \cellcolor[HTML]{F4CCCC}Y \\
\hline
 
\multirow{5}{*}{Wang \etal \cite{wang2018tracking}} & First-gen College Student  & & & & \cellcolor[HTML]{F4CCCC}Y & & & & & & \cellcolor[HTML]{F4CCCC}Y & & \\
  & Gender & & & & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & \\
  & Immigration Status & \cellcolor[HTML]{F4CCCC}Y & & & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & \\
  & Race & & & & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & \\
  & Sexual Orientation & & & & & & & & & & \cellcolor[HTML]{F4CCCC}Y & & \cellcolor[HTML]{F4CCCC}Y \\
\hline

\multirow{5}{*}{Lu \etal \cite{lu2018joint}} & First-gen College Student & \cellcolor[HTML]{F4CCCC}Y & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & & & \\
& Gender & & & & & & & & & & & & \\
& Immigration Status & & & & & & & & & & & & \cellcolor[HTML]{F4CCCC}Y \\
& Race & & \cellcolor[HTML]{F4CCCC}Y & & & & & & & & & & \\
& Sexual Orientation & & & & & & & & & & & & \\
\hline
 
 \multirow{5}{*}{Xu\_interpretable \etal \cite{xu2019leveraging}} & First-gen College Student & & & & & & & & \cellcolor[HTML]{F4CCCC}Y & & & & \\
  & Gender & & & & & & & & & & & & \\
  & Immigration Status & & & & & & & & & & & & \\
  & Race & & & & & & & & & & & & \\
  & Sexual Orientation & & & & & & & & & &  & & \\
\hline
 
 \multirow{5}{*}{Xu\_personalized \etal \cite{xu2021leveraging}} & First-gen College Student & & & & & & & & & & & & \\
  & Gender & & & & & & & & & & & & \\
  & Immigration Status & & & & & & & & & & & & \\
  & Race & & & & \cellcolor[HTML]{F4CCCC}Y & & \cellcolor[HTML]{F4CCCC}Y & & & & & &  \\
  & Sexual Orientation & & & & & & & & & & & \cellcolor[HTML]{F4CCCC}Y & \\
\hline
 
\end{tabular}}
\label{tab_all_w_t_demo}
\end{table}

==> fig_tab_alg/tab_demo.tex <==
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Canzian \etal \cite{canzian2015trajectories} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{F4CCCC}0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.015 & 0.010 \\
 & & Gender & 0.090 & 0.040 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.020 & 0.584 & 0.040 & 0.914 & 0.050 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.014 & \cellcolor[HTML]{F4CCCC}0.020 & 0.061 & 0.030 & 0.933 & 0.050 & 0.878 & 0.040 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.249 & 0.040 & 0.506 & 0.020 & 0.618 & 0.020 \\
 & & Sexual Orientation & 0.216 & 0.050 & 0.568 & 0.050 & 0.561 & 0.030 & 0.667 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.034 & 0.020 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.020 & 0.107 & 0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.063 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.360 & 0.030 & \cellcolor[HTML]{F4CCCC}0.039 & 0.030 \\
 & & Immigration Status & 0.087 & 0.040 & \cellcolor[HTML]{F4CCCC}0.014 & \cellcolor[HTML]{F4CCCC}0.030 & 0.469 & 0.050 & 0.489 & 0.050 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.433 & 0.050 & 0.086 & 0.010 & 0.081 & 0.040 \\
 & & Sexual Orientation & 0.255 & 0.050 & 0.188 & 0.040 & 0.374 & 0.040 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.028 & \cellcolor[HTML]{F4CCCC}0.030 & \cellcolor[HTML]{F4CCCC}0.049 & 0.010 & 0.083 & 0.010 & 0.311 & 0.030 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.041 & 0.040 & 0.439 & 0.050 & 0.239 & 0.020 & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 \\
 & & Immigration Status & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.051 & 0.020 & 0.815 & 0.030 & 0.592 & 0.040 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.020 & 0.057 & 0.030 & 0.937 & 0.040 & \cellcolor[HTML]{F4CCCC}0.025 & 0.020 \\
 & & Sexual Orientation & 0.574 & 0.050 & 0.122 & 0.040 & 0.961 & 0.050 & 0.686 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.034 & 0.020 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.020 & 0.198 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.063 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.360 & 0.020 & \cellcolor[HTML]{F4CCCC}0.031 & 0.030 \\
 & & Immigration Status & 0.087 & 0.040 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.030 & 0.701 & 0.030 & 0.631 & 0.050 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.953 & 0.050 & 0.904 & 0.040 & 0.069 & 0.040 \\
 & & Sexual Orientation & 0.255 & 0.050 & 0.940 & 0.040 & 0.940 & 0.050 & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.028 & \cellcolor[HTML]{F4CCCC}0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.180 & 0.020 & \cellcolor[HTML]{F4CCCC}0.024 & 0.020 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.041 & 0.040 & \cellcolor[HTML]{F4CCCC}0.022 & 0.020 & 0.418 & 0.030 & 0.122 & 0.040 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.017 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{F4CCCC}0.024 & \cellcolor[HTML]{F4CCCC}0.030 & 0.670 & 0.050 & \cellcolor[HTML]{F4CCCC}0.027 & \cellcolor[HTML]{F4CCCC}0.030 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.133 & 0.040 & 0.159 & 0.010 & 0.154 & 0.050 \\
 & & Sexual Orientation & 0.415 & 0.050 & 0.275 & 0.050 & 0.622 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Acc, Canzian.}
\label{tab:appendix_acc_canzian}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Saeb \etal \cite{saeb2015mobile} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.078 & 0.010 & \cellcolor[HTML]{F4CCCC}0.048 & 0.010 \\
 & & Gender & 0.396 & 0.050 & \cellcolor[HTML]{F4CCCC}0.047 & 0.040 & 0.744 & 0.040 & 0.329 & 0.030 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.030 & \cellcolor[HTML]{F4CCCC}0.035 & 0.020 & 0.873 & 0.050 & 0.497 & 0.040 \\
 & & Race & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{F4CCCC}0.045 & 0.030 & 0.201 & 0.020 & 0.182 & 0.020 \\
 & & Sexual Orientation & 0.127 & 0.040 & 0.568 & 0.050 & 0.309 & 0.030 & 0.899 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{F4CCCC}0.045 & 0.020 & 0.094 & 0.010 & 0.096 & 0.040 \\
 & & Gender & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.231 & 0.020 & \cellcolor[HTML]{F4CCCC}0.020 & 0.020 \\
 & & Immigration Status & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.049 & 0.030 & 0.262 & 0.030 & 0.435 & 0.050 \\
 & & Race & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.030 & 0.116 & 0.040 & 0.764 & 0.040 & \cellcolor[HTML]{F4CCCC}0.017 & 0.010 \\
 & & Sexual Orientation & 0.078 & 0.050 & 0.436 & 0.050 & 0.972 & 0.050 & \cellcolor[HTML]{F4CCCC}0.032 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.010 & 0.136 & 0.010 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.032 & \cellcolor[HTML]{F4CCCC}0.040 & 0.092 & 0.020 & 0.247 & 0.020 & 0.130 & 0.040 \\
 & & Immigration Status & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.030 & 0.909 & 0.050 & 0.337 & 0.030 & 0.916 & 0.050 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.020 & 0.097 & 0.030 & 0.892 & 0.050 & 0.050 & 0.030 \\
 & & Sexual Orientation & 0.127 & 0.050 & 0.668 & 0.040 & 0.843 & 0.040 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.030 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & 0.133 & 0.010 & \cellcolor[HTML]{EA9999}0.009 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Gender & 0.389 & 0.040 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.030 & 0.442 & 0.040 & 0.071 & 0.040 \\
 & & Immigration Status & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.147 & 0.020 & 0.683 & 0.050 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.009 & \cellcolor[HTML]{F4CCCC}0.040 & 0.298 & 0.030 & \cellcolor[HTML]{F4CCCC}0.043 & 0.030 \\
 & & Sexual Orientation & 0.766 & 0.050 & 0.292 & 0.050 & 0.870 & 0.050 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & 0.337 & 0.020 & 0.052 & 0.010 \\
 & & Gender & 0.305 & 0.040 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.030 & 0.178 & 0.010 & 0.585 & 0.030 \\
 & & Immigration Status & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.449 & 0.030 & 0.683 & 0.050 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.046 & 0.030 & \cellcolor[HTML]{EA9999}0.009 & \cellcolor[HTML]{F4CCCC}0.040 & 0.655 & 0.040 & 0.487 & 0.020 \\
 & & Sexual Orientation & 0.697 & 0.050 & 0.292 & 0.050 & 0.717 & 0.050 & 0.625 & 0.040 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Acc, Saeb.}
\label{tab:appendix_acc_saeb}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Farhan \etal \cite{farhan2016behavior} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.028 & 0.020 & \cellcolor[HTML]{F4CCCC}0.018 & 0.010 & 0.608 & 0.040 & 0.052 & 0.020 \\
 & & Gender & 0.972 & 0.050 & \cellcolor[HTML]{F4CCCC}0.046 & 0.020 & 0.375 & 0.030 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.218 & 0.030 & 0.283 & 0.030 & 0.190 & 0.020 & 0.433 & 0.040 \\
 & & Race & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.685 & 0.040 & 0.144 & 0.010 & 0.194 & 0.030 \\
 & & Sexual Orientation & 0.497 & 0.040 & 0.909 & 0.050 & 0.645 & 0.050 & 0.518 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.237 & 0.040 & 0.234 & 0.020 & 0.297 & 0.030 & 0.550 & 0.050 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.044 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.171 & 0.020 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.223 & 0.030 & 0.244 & 0.030 & 0.498 & 0.050 & 0.299 & 0.040 \\
 & & Race & 0.145 & 0.020 & 0.516 & 0.050 & 0.058 & 0.010 & 0.124 & 0.020 \\
 & & Sexual Orientation & 0.520 & 0.050 & 0.476 & 0.040 & 0.439 & 0.040 & 0.235 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.735 & 0.040 & 0.195 & 0.030 & 0.641 & 0.040 & 0.067 & 0.030 \\
 & & Gender & 0.074 & 0.010 & \cellcolor[HTML]{F4CCCC}0.016 & \cellcolor[HTML]{F4CCCC}0.020 & 0.146 & 0.030 & \cellcolor[HTML]{F4CCCC}0.050 & 0.010 \\
 & & Immigration Status & 0.229 & 0.030 & 0.403 & 0.040 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.010 & 0.917 & 0.050 \\
 & & Race & 0.225 & 0.020 & 0.544 & 0.050 & 0.050 & 0.020 & 0.236 & 0.040 \\
 & & Sexual Orientation & 0.871 & 0.050 & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.010 & 0.758 & 0.050 & 0.061 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.476 & 0.040 & 0.460 & 0.030 & 0.140 & 0.030 & 0.295 & 0.030 \\
 & & Gender & 0.964 & 0.050 & \cellcolor[HTML]{F4CCCC}0.036 & 0.010 & 0.670 & 0.050 & 0.706 & 0.040 \\
 & & Immigration Status & 0.061 & 0.010 & 0.238 & 0.020 & 0.142 & 0.040 & \cellcolor[HTML]{F4CCCC}0.048 & 0.010 \\
 & & Race & 0.090 & 0.020 & 0.597 & 0.040 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.806 & 0.050 \\
 & & Sexual Orientation & 0.149 & 0.030 & 0.811 & 0.050 & \cellcolor[HTML]{EA9999}0.009 & \cellcolor[HTML]{F4CCCC}0.020 & 0.176 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.856 & 0.050 & 0.372 & 0.040 & 0.492 & 0.030 & 0.596 & 0.050 \\
 & & Gender & 0.685 & 0.040 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 & 0.175 & 0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.626 & 0.030 & 0.716 & 0.050 & 0.696 & 0.040 & 0.137 & 0.030 \\
 & & Race & 0.058 & 0.010 & 0.330 & 0.030 & 0.758 & 0.050 & 0.109 & 0.020 \\
 & & Sexual Orientation & 0.328 & 0.020 & 0.068 & 0.020 & \cellcolor[HTML]{F4CCCC}0.037 & 0.010 & 0.143 & 0.040 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Acc, Farhan.}
\label{tab:appendix_acc_farhan}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Wahle \etal \cite{wahle2016mobile} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.020 & 0.118 & 0.020 & \cellcolor[HTML]{EA9999}0.010 & \cellcolor[HTML]{F4CCCC}0.010 & 0.066 & 0.010 \\
 & & Gender & 0.311 & 0.050 & \cellcolor[HTML]{F4CCCC}0.017 & 0.010 & 0.894 & 0.050 & 0.496 & 0.030 \\
 & & Immigration Status & 0.074 & 0.030 & 0.198 & 0.040 & 0.466 & 0.030 & 0.084 & 0.020 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.174 & 0.030 & 0.482 & 0.040 & 0.749 & 0.040 \\
 & & Sexual Orientation & 0.198 & 0.040 & 0.459 & 0.050 & 0.220 & 0.020 & 0.946 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & 0.622 & 0.040 & 0.857 & 0.040 \\
 & & Gender & 0.203 & 0.050 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.054 & 0.010 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.038 & 0.030 & 0.061 & 0.030 & 0.222 & 0.020 & 0.707 & 0.030 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.114 & 0.040 & 0.348 & 0.030 & 0.970 & 0.050 \\
 & & Sexual Orientation & 0.198 & 0.040 & 0.568 & 0.050 & 0.764 & 0.050 & 0.707 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.885 & 0.050 & 0.057 & 0.010 \\
 & & Gender & 0.352 & 0.050 & \cellcolor[HTML]{F4CCCC}0.037 & 0.020 & 0.766 & 0.040 & 0.472 & 0.040 \\
 & & Immigration Status & 0.064 & 0.030 & 0.515 & 0.030 & 0.319 & 0.010 & 0.854 & 0.050 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.938 & 0.050 & 0.633 & 0.020 & 0.418 & 0.030 \\
 & & Sexual Orientation & 0.182 & 0.040 & 0.656 & 0.040 & 0.671 & 0.030 & 0.152 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{F4CCCC}0.048 & 0.010 & 0.308 & 0.010 & 0.298 & 0.030 \\
 & & Gender & 0.352 & 0.050 & 0.059 & 0.020 & 0.955 & 0.050 & 0.926 & 0.050 \\
 & & Immigration Status & 0.064 & 0.030 & 0.581 & 0.030 & 0.352 & 0.020 & 0.700 & 0.040 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.934 & 0.050 & 0.504 & 0.040 & 0.243 & 0.010 \\
 & & Sexual Orientation & 0.331 & 0.040 & 0.628 & 0.040 & 0.479 & 0.030 & 0.262 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.446 & 0.030 & 0.082 & 0.010 \\
 & & Gender & 0.311 & 0.050 & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.020 & 0.470 & 0.040 & 0.970 & 0.050 \\
 & & Immigration Status & 0.074 & 0.030 & \cellcolor[HTML]{F4CCCC}0.031 & 0.030 & 0.087 & 0.020 & 0.561 & 0.020 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.115 & 0.040 & 0.087 & 0.010 & 0.611 & 0.030 \\
 & & Sexual Orientation & 0.198 & 0.040 & 0.387 & 0.050 & 0.847 & 0.050 & 0.691 & 0.040 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Acc, Wahle.}
\label{tab:appendix_acc_wahle}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Lu \etal \cite{lu2018joint} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.824 & 0.050 & 0.692 & 0.040 & 0.460 & 0.050 \\
 & & Gender & 0.251 & 0.030 & 0.376 & 0.040 & 0.987 & 0.050 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.622 & 0.050 & 0.216 & 0.020 & 0.480 & 0.030 & 0.068 & 0.030 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.018 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.113 & 0.010 & 0.151 & 0.040 \\
 & & Sexual Orientation & 0.509 & 0.040 & 0.300 & 0.030 & 0.212 & 0.020 & \cellcolor[HTML]{F4CCCC}0.015 & \cellcolor[HTML]{F4CCCC}0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.015 & 0.010 & 0.886 & 0.050 & 0.967 & 0.050 & 0.943 & 0.040 \\
 & & Gender & 0.067 & 0.020 & 0.503 & 0.030 & 0.216 & 0.020 & 0.202 & 0.010 \\
 & & Immigration Status & 0.985 & 0.050 & 0.854 & 0.040 & 0.544 & 0.040 & 0.854 & 0.030 \\
 & & Race & 0.125 & 0.030 & 0.225 & 0.010 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.271 & 0.020 \\
 & & Sexual Orientation & 0.538 & 0.040 & 0.235 & 0.020 & 0.427 & 0.030 & 0.951 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.325 & 0.040 & \cellcolor[HTML]{F4CCCC}0.018 & 0.010 & 0.616 & 0.040 \\
 & & Gender & 0.895 & 0.050 & 0.092 & 0.030 & 0.148 & 0.030 & 0.186 & 0.010 \\
 & & Immigration Status & 0.120 & 0.030 & 0.559 & 0.050 & 0.353 & 0.040 & 0.373 & 0.030 \\
 & & Race & 0.061 & 0.020 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.042 & 0.020 & 0.791 & 0.050 \\
 & & Sexual Orientation & 0.363 & 0.040 & \cellcolor[HTML]{F4CCCC}0.026 & 0.020 & 0.715 & 0.050 & 0.336 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.134 & 0.030 & 0.207 & 0.040 & 0.768 & 0.040 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.115 & 0.020 & \cellcolor[HTML]{F4CCCC}0.035 & 0.010 & 0.543 & 0.030 & 0.328 & 0.030 \\
 & & Immigration Status & 0.314 & 0.040 & 0.379 & 0.050 & 0.934 & 0.050 & 0.108 & 0.020 \\
 & & Race & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.046 & 0.020 & 0.088 & 0.010 & 0.498 & 0.040 \\
 & & Sexual Orientation & 0.481 & 0.050 & 0.113 & 0.030 & 0.089 & 0.020 & 0.994 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.083 & 0.020 & 0.082 & 0.020 & 0.511 & 0.030 & 0.326 & 0.040 \\
 & & Gender & 0.289 & 0.040 & 0.365 & 0.040 & 0.111 & 0.010 & \cellcolor[HTML]{F4CCCC}0.031 & 0.020 \\
 & & Immigration Status & 0.806 & 0.050 & 0.620 & 0.050 & 0.930 & 0.050 & \cellcolor[HTML]{F4CCCC}0.016 & 0.010 \\
 & & Race & 0.147 & 0.030 & 0.319 & 0.030 & 0.181 & 0.020 & 0.476 & 0.050 \\
 & & Sexual Orientation & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.038 & 0.010 & 0.689 & 0.040 & 0.298 & 0.030 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Acc, Lu.}
\label{tab:appendix_acc_lu}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Wang \etal \cite{wang2018tracking} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & 0.105 & 0.030 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.924 & 0.050 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.030 & 0.642 & 0.050 & 0.743 & 0.050 \\
 & & Immigration Status & 0.179 & 0.020 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.258 & 0.040 & 0.457 & 0.030 \\
 & & Race & 0.183 & 0.030 & \cellcolor[HTML]{F4CCCC}0.012 & \cellcolor[HTML]{F4CCCC}0.040 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 & 0.734 & 0.040 \\
 & & Sexual Orientation & 0.728 & 0.040 & 0.307 & 0.050 & \cellcolor[HTML]{F4CCCC}0.030 & 0.020 & \cellcolor[HTML]{F4CCCC}0.038 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.411 & 0.050 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{F4CCCC}0.015 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.207 & 0.020 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.030 & 0.418 & 0.050 & \cellcolor[HTML]{F4CCCC}0.016 & \cellcolor[HTML]{F4CCCC}0.030 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.123 & 0.030 & 0.663 & 0.050 \\
 & & Race & 0.363 & 0.040 & \cellcolor[HTML]{F4CCCC}0.012 & \cellcolor[HTML]{F4CCCC}0.040 & \cellcolor[HTML]{F4CCCC}0.016 & \cellcolor[HTML]{F4CCCC}0.020 & 0.170 & 0.040 \\
 & & Sexual Orientation & 0.335 & 0.030 & 0.307 & 0.050 & 0.141 & 0.040 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.018 & 0.010 & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.030 & \cellcolor[HTML]{F4CCCC}0.015 & 0.010 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.061 & 0.040 & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.020 & 0.418 & 0.050 & 0.164 & 0.040 \\
 & & Immigration Status & 0.055 & 0.030 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.123 & 0.030 & 0.824 & 0.050 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.021 & 0.020 & \cellcolor[HTML]{F4CCCC}0.021 & \cellcolor[HTML]{F4CCCC}0.040 & \cellcolor[HTML]{F4CCCC}0.016 & \cellcolor[HTML]{F4CCCC}0.020 & 0.073 & 0.030 \\
 & & Sexual Orientation & 0.097 & 0.050 & 0.307 & 0.050 & 0.141 & 0.040 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.018 & 0.010 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{F4CCCC}0.031 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.806 & 0.040 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.030 & 0.418 & 0.050 & \cellcolor[HTML]{F4CCCC}0.016 & \cellcolor[HTML]{F4CCCC}0.030 \\
 & & Immigration Status & 0.187 & 0.030 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.067 & 0.030 & 0.663 & 0.050 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.040 & 0.020 & \cellcolor[HTML]{F4CCCC}0.012 & \cellcolor[HTML]{F4CCCC}0.040 & \cellcolor[HTML]{F4CCCC}0.032 & 0.020 & 0.170 & 0.040 \\
 & & Sexual Orientation & 0.838 & 0.050 & 0.307 & 0.050 & 0.141 & 0.040 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.036 & 0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.777 & 0.040 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.030 & 0.485 & 0.050 & \cellcolor[HTML]{F4CCCC}0.016 & \cellcolor[HTML]{F4CCCC}0.030 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.026 & 0.010 & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.108 & 0.030 & 0.663 & 0.050 \\
 & & Race & 0.465 & 0.030 & \cellcolor[HTML]{F4CCCC}0.012 & \cellcolor[HTML]{F4CCCC}0.040 & \cellcolor[HTML]{F4CCCC}0.013 & 0.010 & 0.170 & 0.040 \\
 & & Sexual Orientation & 0.867 & 0.050 & 0.307 & 0.050 & 0.128 & 0.040 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.020 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Acc, Wang.}
\label{tab:appendix_acc_wang}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Xu\_interpretable \etal \cite{xu2019leveraging} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.250 & 0.030 & 0.120 & 0.020 & 0.792 & 0.040 & 0.335 & 0.030 \\
 & & Gender & 0.082 & 0.010 & 0.099 & 0.010 & 0.422 & 0.020 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.325 & 0.050 & 0.584 & 0.050 & 0.446 & 0.030 & 0.630 & 0.040 \\
 & & Race & 0.281 & 0.040 & 0.329 & 0.040 & 0.074 & 0.010 & 0.311 & 0.020 \\
 & & Sexual Orientation & 0.238 & 0.020 & 0.268 & 0.030 & 0.905 & 0.050 & 0.781 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.250 & 0.030 & 0.212 & 0.010 & 0.221 & 0.010 & 0.615 & 0.050 \\
 & & Gender & 0.082 & 0.010 & 0.507 & 0.030 & 0.241 & 0.020 & 0.350 & 0.020 \\
 & & Immigration Status & 0.325 & 0.050 & 0.965 & 0.050 & 0.573 & 0.050 & 0.421 & 0.030 \\
 & & Race & 0.281 & 0.040 & 0.441 & 0.020 & 0.552 & 0.040 & 0.348 & 0.010 \\
 & & Sexual Orientation & 0.238 & 0.020 & 0.936 & 0.040 & 0.314 & 0.030 & 0.531 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.250 & 0.030 & 0.242 & 0.030 & 0.221 & 0.010 & 0.335 & 0.030 \\
 & & Gender & 0.082 & 0.010 & 0.078 & 0.020 & 0.241 & 0.020 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.325 & 0.050 & \cellcolor[HTML]{F4CCCC}0.027 & 0.010 & 0.573 & 0.050 & 0.630 & 0.040 \\
 & & Race & 0.281 & 0.040 & 0.634 & 0.040 & 0.552 & 0.040 & 0.311 & 0.020 \\
 & & Sexual Orientation & 0.238 & 0.020 & 0.804 & 0.050 & 0.314 & 0.030 & 0.781 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.250 & 0.030 & 0.167 & 0.020 & 0.221 & 0.010 & 0.335 & 0.030 \\
 & & Gender & 0.082 & 0.010 & 0.095 & 0.010 & 0.241 & 0.020 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.325 & 0.050 & 0.636 & 0.050 & 0.573 & 0.050 & 0.630 & 0.040 \\
 & & Race & 0.281 & 0.040 & 0.382 & 0.030 & 0.552 & 0.040 & 0.311 & 0.020 \\
 & & Sexual Orientation & 0.238 & 0.020 & 0.584 & 0.040 & 0.314 & 0.030 & 0.781 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.250 & 0.030 & 0.242 & 0.030 & 0.221 & 0.010 & 0.335 & 0.030 \\
 & & Gender & 0.082 & 0.010 & 0.078 & 0.020 & 0.241 & 0.020 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.325 & 0.050 & \cellcolor[HTML]{F4CCCC}0.027 & 0.010 & 0.573 & 0.050 & 0.630 & 0.040 \\
 & & Race & 0.281 & 0.040 & 0.634 & 0.040 & 0.552 & 0.040 & 0.311 & 0.020 \\
 & & Sexual Orientation & 0.238 & 0.020 & 0.804 & 0.050 & 0.314 & 0.030 & 0.781 & 0.050 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Acc, Xu\_interpretable.}
\label{tab:appendix_acc_xu_interpretable}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Xu\_personalized \etal \cite{xu2021leveraging} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.728 & 0.040 & \cellcolor[HTML]{F4CCCC}0.039 & 0.020 & 0.696 & 0.030 & 0.294 & 0.020 \\
 & & Gender & 0.218 & 0.010 & 0.318 & 0.040 & 0.910 & 0.050 & 0.842 & 0.050 \\
 & & Immigration Status & 0.904 & 0.050 & 0.129 & 0.030 & 0.185 & 0.010 & 0.629 & 0.040 \\
 & & Race & 0.421 & 0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.396 & 0.020 & 0.343 & 0.030 \\
 & & Sexual Orientation & 0.547 & 0.030 & 0.826 & 0.050 & 0.825 & 0.040 & 0.066 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.728 & 0.040 & \cellcolor[HTML]{F4CCCC}0.039 & 0.020 & 0.696 & 0.030 & 0.294 & 0.020 \\
 & & Gender & 0.218 & 0.010 & 0.318 & 0.040 & 0.910 & 0.050 & 0.842 & 0.050 \\
 & & Immigration Status & 0.904 & 0.050 & 0.129 & 0.030 & 0.185 & 0.010 & 0.629 & 0.040 \\
 & & Race & 0.421 & 0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.396 & 0.020 & 0.343 & 0.030 \\
 & & Sexual Orientation & 0.547 & 0.030 & 0.826 & 0.050 & 0.825 & 0.040 & 0.066 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.728 & 0.040 & \cellcolor[HTML]{F4CCCC}0.039 & 0.020 & 0.696 & 0.030 & 0.294 & 0.020 \\
 & & Gender & 0.218 & 0.010 & 0.318 & 0.040 & 0.910 & 0.050 & 0.842 & 0.050 \\
 & & Immigration Status & 0.904 & 0.050 & 0.129 & 0.030 & 0.185 & 0.010 & 0.629 & 0.040 \\
 & & Race & 0.421 & 0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.396 & 0.020 & 0.343 & 0.030 \\
 & & Sexual Orientation & 0.547 & 0.030 & 0.826 & 0.050 & 0.825 & 0.040 & 0.066 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.728 & 0.040 & \cellcolor[HTML]{F4CCCC}0.039 & 0.020 & 0.696 & 0.030 & 0.294 & 0.020 \\
 & & Gender & 0.218 & 0.010 & 0.318 & 0.040 & 0.910 & 0.050 & 0.842 & 0.050 \\
 & & Immigration Status & 0.904 & 0.050 & 0.129 & 0.030 & 0.185 & 0.010 & 0.629 & 0.040 \\
 & & Race & 0.421 & 0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.396 & 0.020 & 0.343 & 0.030 \\
 & & Sexual Orientation & 0.547 & 0.030 & 0.826 & 0.050 & 0.825 & 0.040 & 0.066 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.728 & 0.040 & \cellcolor[HTML]{F4CCCC}0.039 & 0.020 & 0.696 & 0.030 & 0.294 & 0.020 \\
 & & Gender & 0.218 & 0.010 & 0.318 & 0.040 & 0.910 & 0.050 & 0.842 & 0.050 \\
 & & Immigration Status & 0.904 & 0.050 & 0.129 & 0.030 & 0.185 & 0.010 & 0.629 & 0.040 \\
 & & Race & 0.421 & 0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.396 & 0.020 & 0.343 & 0.030 \\
 & & Sexual Orientation & 0.547 & 0.030 & 0.826 & 0.050 & 0.825 & 0.040 & 0.066 & 0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Acc, Xu\_personalized.}
\label{tab:appendix_acc_xu_personalized}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Canzian \etal \cite{canzian2015trajectories} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.120 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.354 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.240 & 0.040 & 0.567 & 0.040 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.037 & 0.030 \\
 & & Immigration Status & 0.216 & 0.030 & 0.623 & 0.050 & 0.256 & 0.020 & 0.580 & 0.040 \\
 & & Race & 0.123 & 0.020 & 0.348 & 0.030 & 0.461 & 0.050 & \cellcolor[HTML]{F4CCCC}0.021 & 0.020 \\
 & & Sexual Orientation & 0.389 & 0.050 & \cellcolor[HTML]{F4CCCC}0.042 & 0.020 & 0.357 & 0.040 & 0.753 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}0.016 & 0.010 & 0.173 & 0.020 & 0.070 & 0.030 \\
 & & Gender & 1.000 & 0.030 & 0.200 & 0.020 & 0.731 & 0.030 & 0.068 & 0.020 \\
 & & Immigration Status & 1.000 & 0.030 & 0.949 & 0.050 & 0.769 & 0.040 & 0.614 & 0.040 \\
 & & Race & 1.000 & 0.030 & 0.590 & 0.030 & 0.819 & 0.050 & \cellcolor[HTML]{F4CCCC}0.024 & 0.010 \\
 & & Sexual Orientation & 1.000 & 0.030 & 0.898 & 0.040 & 0.108 & 0.010 & 0.847 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.771 & 0.040 & 0.992 & 0.050 & 0.098 & 0.020 & 0.473 & 0.050 \\
 & & Gender & 0.175 & 0.030 & 0.789 & 0.040 & \cellcolor[HTML]{F4CCCC}0.019 & 0.010 & 0.126 & 0.040 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.315 & 0.040 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Race & 0.792 & 0.050 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.020 & 0.263 & 0.030 & \cellcolor[HTML]{F4CCCC}0.041 & 0.030 \\
 & & Sexual Orientation & 0.115 & 0.020 & 0.783 & 0.030 & 0.416 & 0.050 & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 1.000 & 0.030 & 0.197 & 0.030 & 0.888 & 0.040 & \cellcolor[HTML]{F4CCCC}0.017 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Gender & 1.000 & 0.030 & 0.770 & 0.050 & 0.241 & 0.030 & 0.093 & 0.030 \\
 & & Immigration Status & 1.000 & 0.030 & 0.216 & 0.040 & 0.139 & 0.010 & 0.450 & 0.040 \\
 & & Race & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}0.037 & 0.010 & 0.971 & 0.050 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Sexual Orientation & 1.000 & 0.030 & 0.142 & 0.020 & 0.229 & 0.020 & 0.653 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.036 & 0.020 & 0.531 & 0.040 & 0.367 & 0.030 & 0.655 & 0.050 \\
 & & Gender & 0.281 & 0.050 & 0.799 & 0.050 & 0.241 & 0.020 & 0.115 & 0.020 \\
 & & Immigration Status & 0.095 & 0.040 & 0.488 & 0.030 & 0.585 & 0.040 & 0.116 & 0.030 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.010 & 0.010 & 0.224 & 0.020 & 0.971 & 0.050 & 0.644 & 0.040 \\
 & & Sexual Orientation & \cellcolor[HTML]{F4CCCC}0.043 & 0.030 & 0.162 & 0.010 & 0.229 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fnr, Canzian.}
\label{tab:appendix_fnr_canzian}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Saeb \etal \cite{saeb2015mobile} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.782 & 0.050 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.611 & 0.040 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{F4CCCC}0.030 & 0.348 & 0.040 & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.030 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.730 & 0.050 & 0.855 & 0.050 & 0.395 & 0.050 \\
 & & Race & 0.232 & 0.030 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.020 & 0.102 & 0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Sexual Orientation & 0.052 & 0.020 & 0.605 & 0.040 & 0.165 & 0.030 & 0.338 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.537 & 0.040 & 0.275 & 0.020 & 0.604 & 0.030 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.849 & 0.050 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.826 & 0.050 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 & 0.895 & 0.050 & 0.585 & 0.020 & 0.531 & 0.050 \\
 & & Race & 0.275 & 0.030 & 0.579 & 0.030 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 & 0.082 & 0.040 \\
 & & Sexual Orientation & 0.053 & 0.020 & 0.790 & 0.040 & 0.705 & 0.040 & \cellcolor[HTML]{F4CCCC}0.024 & \cellcolor[HTML]{F4CCCC}0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.210 & 0.030 & 0.179 & 0.030 & 0.527 & 0.040 & 0.119 & 0.030 \\
 & & Gender & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 & 0.883 & 0.050 & 0.244 & 0.020 & 0.416 & 0.040 \\
 & & Immigration Status & 0.404 & 0.050 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.536 & 0.050 & 1.000 & 0.050 \\
 & & Race & 0.232 & 0.040 & \cellcolor[HTML]{F4CCCC}0.031 & 0.020 & \cellcolor[HTML]{F4CCCC}0.019 & 0.010 & 0.060 & 0.020 \\
 & & Sexual Orientation & 0.052 & 0.020 & 0.539 & 0.040 & 0.489 & 0.030 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.982 & 0.050 & 1.000 & 0.030 & 0.968 & 0.040 & \cellcolor[HTML]{F4CCCC}0.042 & 0.030 \\
 & & Gender & 0.570 & 0.030 & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}0.041 & 0.010 & 0.416 & 0.040 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.020 & 1.000 & 0.030 & 0.983 & 0.050 & 0.583 & 0.050 \\
 & & Race & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 & 1.000 & 0.030 & 0.437 & 0.020 & \cellcolor[HTML]{F4CCCC}0.014 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Sexual Orientation & 0.643 & 0.040 & 1.000 & 0.030 & 0.649 & 0.030 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.156 & 0.030 & 1.000 & 0.030 & 0.541 & 0.040 & 0.460 & 0.040 \\
 & & Gender & 0.722 & 0.050 & 1.000 & 0.030 & 0.774 & 0.050 & \cellcolor[HTML]{F4CCCC}0.032 & 0.020 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & 1.000 & 0.030 & 0.412 & 0.030 & 0.921 & 0.050 \\
 & & Race & 0.196 & 0.040 & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}0.010 & 0.010 & 0.052 & 0.030 \\
 & & Sexual Orientation & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 1.000 & 0.030 & 0.218 & 0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fnr, Saeb.}
\label{tab:appendix_fnr_saeb}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Farhan \etal \cite{farhan2016behavior} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.476 & 0.040 & 0.253 & 0.020 & 0.139 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.113 & 0.030 & 0.860 & 0.050 & 0.657 & 0.050 & 0.471 & 0.040 \\
 & & Immigration Status & 0.056 & 0.020 & 0.162 & 0.010 & 0.264 & 0.030 & 1.000 & 0.050 \\
 & & Race & 0.988 & 0.050 & 0.545 & 0.040 & 0.260 & 0.020 & 0.113 & 0.020 \\
 & & Sexual Orientation & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.494 & 0.030 & 0.322 & 0.040 & 0.143 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.990 & 0.050 & 0.502 & 0.040 & 0.337 & 0.020 & 0.842 & 0.040 \\
 & & Gender & 0.363 & 0.020 & 0.085 & 0.020 & 0.156 & 0.010 & 0.583 & 0.020 \\
 & & Immigration Status & 0.268 & 0.010 & \cellcolor[HTML]{F4CCCC}0.036 & 0.010 & 0.909 & 0.050 & 0.780 & 0.030 \\
 & & Race & 0.656 & 0.040 & 0.353 & 0.030 & 0.619 & 0.040 & 0.102 & 0.010 \\
 & & Sexual Orientation & 0.398 & 0.030 & 0.880 & 0.050 & 0.575 & 0.030 & 0.894 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.477 & 0.040 & 0.635 & 0.050 & 0.457 & 0.030 & \cellcolor[HTML]{F4CCCC}0.025 & 0.010 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.014 & \cellcolor[HTML]{F4CCCC}0.020 & 0.146 & 0.030 & 0.768 & 0.040 & 0.903 & 0.050 \\
 & & Immigration Status & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.010 & 0.092 & 0.020 \\
 & & Race & 0.053 & 0.030 & 0.301 & 0.040 & \cellcolor[HTML]{F4CCCC}0.028 & 0.020 & 0.138 & 0.030 \\
 & & Sexual Orientation & 0.816 & 0.050 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & 0.937 & 0.050 & 0.374 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.174 & 0.020 & 0.479 & 0.040 & 0.618 & 0.050 & \cellcolor[HTML]{F4CCCC}0.037 & 0.010 \\
 & & Gender & 0.255 & 0.030 & 0.569 & 0.050 & 0.503 & 0.040 & 0.781 & 0.050 \\
 & & Immigration Status & 0.400 & 0.040 & 0.388 & 0.030 & \cellcolor[HTML]{F4CCCC}0.046 & 0.020 & 0.632 & 0.030 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.028 & 0.010 & 0.225 & 0.020 & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & 0.102 & 0.020 \\
 & & Sexual Orientation & 0.655 & 0.050 & 0.222 & 0.010 & 0.054 & 0.030 & 0.706 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.912 & 0.050 & 0.842 & 0.040 & 0.475 & 0.040 & 0.156 & 0.010 \\
 & & Gender & 0.804 & 0.040 & 0.061 & 0.030 & 0.407 & 0.030 & 0.402 & 0.020 \\
 & & Immigration Status & 0.575 & 0.030 & \cellcolor[HTML]{F4CCCC}0.014 & \cellcolor[HTML]{F4CCCC}0.020 & 0.844 & 0.050 & 0.632 & 0.040 \\
 & & Race & 0.323 & 0.020 & 0.949 & 0.050 & \cellcolor[HTML]{F4CCCC}0.043 & 0.010 & 0.684 & 0.050 \\
 & & Sexual Orientation & 0.157 & 0.010 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 & 0.064 & 0.020 & 0.450 & 0.030 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fnr, Farhan.}
\label{tab:appendix_fnr_farhan}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Wahle \etal \cite{wahle2016mobile} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.845 & 0.050 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.865 & 0.050 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.618 & 0.040 & 0.407 & 0.040 & 0.084 & 0.010 & 0.495 & 0.030 \\
 & & Immigration Status & 0.124 & 0.010 & 0.346 & 0.030 & 0.562 & 0.040 & 0.777 & 0.040 \\
 & & Race & 0.219 & 0.020 & 0.233 & 0.020 & 0.486 & 0.030 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Sexual Orientation & 0.284 & 0.030 & 0.534 & 0.050 & 0.103 & 0.020 & 0.986 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.630 & 0.050 & 0.206 & 0.030 & 0.349 & 0.020 & 0.077 & 0.010 \\
 & & Gender & 0.489 & 0.040 & 0.189 & 0.020 & 0.320 & 0.010 & 0.433 & 0.020 \\
 & & Immigration Status & 0.095 & 0.010 & 0.998 & 0.050 & 0.926 & 0.050 & 0.781 & 0.050 \\
 & & Race & 0.181 & 0.020 & 0.876 & 0.040 & 0.433 & 0.030 & 0.589 & 0.030 \\
 & & Sexual Orientation & 0.244 & 0.030 & 0.068 & 0.010 & 0.592 & 0.040 & 0.774 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.845 & 0.050 & 0.847 & 0.050 & 0.469 & 0.020 & 0.278 & 0.030 \\
 & & Gender & 0.618 & 0.040 & 0.246 & 0.030 & 0.469 & 0.020 & 0.678 & 0.050 \\
 & & Immigration Status & 0.124 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.346 & 0.010 & \cellcolor[HTML]{F4CCCC}0.014 & 0.010 \\
 & & Race & 0.219 & 0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & 0.723 & 0.040 & \cellcolor[HTML]{F4CCCC}0.047 & 0.020 \\
 & & Sexual Orientation & 0.284 & 0.030 & 0.752 & 0.040 & 0.738 & 0.050 & 0.541 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.758 & 0.050 & 0.179 & 0.020 & 0.773 & 0.030 & 0.347 & 0.020 \\
 & & Gender & 0.489 & 0.040 & 0.334 & 0.040 & 0.141 & 0.010 & 0.517 & 0.050 \\
 & & Immigration Status & 0.095 & 0.010 & 0.875 & 0.050 & 0.989 & 0.050 & 0.454 & 0.040 \\
 & & Race & 0.181 & 0.020 & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & 0.790 & 0.040 & \cellcolor[HTML]{F4CCCC}0.034 & 0.010 \\
 & & Sexual Orientation & 0.244 & 0.030 & 0.211 & 0.030 & 0.494 & 0.020 & 0.438 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.845 & 0.050 & 0.305 & 0.030 & 0.997 & 0.050 & 0.439 & 0.030 \\
 & & Gender & 0.618 & 0.040 & 0.250 & 0.020 & 0.117 & 0.010 & 0.361 & 0.020 \\
 & & Immigration Status & 0.124 & 0.010 & 0.904 & 0.040 & 0.246 & 0.020 & 0.927 & 0.040 \\
 & & Race & 0.219 & 0.020 & 0.960 & 0.050 & 0.449 & 0.030 & 0.969 & 0.050 \\
 & & Sexual Orientation & 0.284 & 0.030 & 0.063 & 0.010 & 0.896 & 0.040 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fnr, Wahle.}
\label{tab:appendix_fnr_wahle}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Lu \etal \cite{lu2018joint} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.579 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.397 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.216 & 0.020 & 0.951 & 0.040 & 0.951 & 0.050 & \cellcolor[HTML]{EA9999}0.009 & \cellcolor[HTML]{F4CCCC}0.030 \\
 & & Immigration Status & 0.752 & 0.050 & 0.358 & 0.030 & 0.162 & 0.030 & 0.351 & 0.050 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.046 & 0.020 & 0.151 & 0.020 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Sexual Orientation & 0.652 & 0.040 & 1.000 & 0.050 & 0.102 & 0.010 & 0.297 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.029 & \cellcolor[HTML]{F4CCCC}0.030 & 0.156 & 0.020 & 0.474 & 0.040 & 0.271 & 0.040 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.012 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.746 & 0.050 & 0.051 & 0.010 \\
 & & Immigration Status & 0.912 & 0.050 & 0.908 & 0.050 & 0.062 & 0.020 & 0.090 & 0.030 \\
 & & Race & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 & 0.478 & 0.030 & \cellcolor[HTML]{F4CCCC}0.019 & 0.010 & 0.085 & 0.020 \\
 & & Sexual Orientation & 0.816 & 0.040 & 0.621 & 0.040 & 0.102 & 0.030 & 0.693 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.186 & 0.040 & 0.060 & 0.030 & 0.377 & 0.020 & 0.076 & 0.010 \\
 & & Gender & 0.828 & 0.050 & \cellcolor[HTML]{F4CCCC}0.019 & \cellcolor[HTML]{F4CCCC}0.020 & 0.633 & 0.050 & 0.155 & 0.020 \\
 & & Immigration Status & 0.118 & 0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.456 & 0.040 & 0.611 & 0.050 \\
 & & Race & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.565 & 0.050 & 0.387 & 0.030 & 0.175 & 0.030 \\
 & & Sexual Orientation & 0.147 & 0.030 & 0.247 & 0.040 & 0.252 & 0.010 & 0.463 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.418 & 0.030 & \cellcolor[HTML]{F4CCCC}0.030 & 0.020 & 0.375 & 0.030 & 0.233 & 0.020 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.021 & 0.020 & 0.131 & 0.040 & 0.375 & 0.030 & 0.571 & 0.040 \\
 & & Immigration Status & 0.989 & 0.050 & \cellcolor[HTML]{F4CCCC}0.030 & 0.030 & \cellcolor[HTML]{F4CCCC}0.025 & 0.020 & 0.944 & 0.050 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Sexual Orientation & 0.791 & 0.040 & 0.851 & 0.050 & 0.868 & 0.050 & 0.562 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.058 & 0.020 & 0.207 & 0.030 & 0.831 & 0.050 & 0.661 & 0.040 \\
 & & Gender & 0.665 & 0.040 & 0.537 & 0.050 & \cellcolor[HTML]{F4CCCC}0.034 & 0.010 & 0.050 & 0.010 \\
 & & Immigration Status & 0.441 & 0.030 & 0.107 & 0.020 & 0.090 & 0.020 & 0.654 & 0.030 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.486 & 0.040 & 0.518 & 0.040 & 0.745 & 0.050 \\
 & & Sexual Orientation & 0.952 & 0.050 & 0.052 & 0.010 & 0.112 & 0.030 & 0.579 & 0.020 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fnr, Lu.}
\label{tab:appendix_fnr_lu}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Wang \etal \cite{wang2018tracking} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.281 & 0.020 & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}0.014 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.480 & 0.030 & 1.000 & 0.030 & 0.826 & 0.050 & 0.207 & 0.040 \\
 & & Immigration Status & 0.949 & 0.050 & 1.000 & 0.030 & 0.598 & 0.030 & 0.514 & 0.050 \\
 & & Race & 0.079 & 0.010 & 1.000 & 0.030 & 0.071 & 0.020 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Sexual Orientation & 0.571 & 0.040 & 1.000 & 0.030 & 0.747 & 0.040 & 0.058 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.243 & 0.020 & 1.000 & 0.030 & 0.982 & 0.050 & 1.000 & 0.030 \\
 & & Gender & 0.568 & 0.040 & 1.000 & 0.030 & 0.647 & 0.040 & 1.000 & 0.030 \\
 & & Immigration Status & 0.407 & 0.030 & 1.000 & 0.030 & 0.441 & 0.020 & 1.000 & 0.030 \\
 & & Race & 0.053 & 0.010 & 1.000 & 0.030 & 0.097 & 0.010 & 1.000 & 0.030 \\
 & & Sexual Orientation & 0.717 & 0.050 & 1.000 & 0.030 & 0.607 & 0.030 & 1.000 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.856 & 0.050 & 0.072 & 0.020 & 0.982 & 0.050 & 0.196 & 0.020 \\
 & & Gender & 0.063 & 0.010 & 0.234 & 0.030 & 0.647 & 0.040 & \cellcolor[HTML]{F4CCCC}0.024 & 0.010 \\
 & & Immigration Status & 0.585 & 0.040 & 0.052 & 0.010 & 0.441 & 0.020 & 0.959 & 0.050 \\
 & & Race & 0.103 & 0.020 & 0.404 & 0.040 & 0.097 & 0.010 & 0.771 & 0.040 \\
 & & Sexual Orientation & 0.156 & 0.030 & 0.735 & 0.050 & 0.607 & 0.030 & 0.237 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.477 & 0.030 & 1.000 & 0.030 & 0.927 & 0.040 & 1.000 & 0.030 \\
 & & Gender & 0.666 & 0.040 & 1.000 & 0.030 & 0.398 & 0.020 & 1.000 & 0.030 \\
 & & Immigration Status & 0.880 & 0.050 & 1.000 & 0.030 & 0.290 & 0.010 & 1.000 & 0.030 \\
 & & Race & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 1.000 & 0.030 & 0.426 & 0.030 & 1.000 & 0.030 \\
 & & Sexual Orientation & 0.332 & 0.020 & 1.000 & 0.030 & 0.995 & 0.050 & 1.000 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.799 & 0.050 & 1.000 & 0.030 & 0.982 & 0.050 & 1.000 & 0.030 \\
 & & Gender & 0.348 & 0.030 & 1.000 & 0.030 & 0.647 & 0.040 & 1.000 & 0.030 \\
 & & Immigration Status & 0.738 & 0.040 & 1.000 & 0.030 & 0.441 & 0.020 & 1.000 & 0.030 \\
 & & Race & 0.053 & 0.010 & 1.000 & 0.030 & 0.097 & 0.010 & 1.000 & 0.030 \\
 & & Sexual Orientation & 0.115 & 0.020 & 1.000 & 0.030 & 0.607 & 0.030 & 1.000 & 0.030 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fnr, Wang.}
\label{tab:appendix_fnr_wang}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Xu\_interpretable \etal \cite{xu2019leveraging} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.874 & 0.040 & 0.516 & 0.020 & 0.321 & 0.030 & 0.304 & 0.020 \\
 & & Gender & 0.186 & 0.010 & 0.673 & 0.030 & 0.887 & 0.050 & 0.964 & 0.050 \\
 & & Immigration Status & 0.719 & 0.030 & 0.821 & 0.050 & 0.392 & 0.040 & 0.517 & 0.040 \\
 & & Race & 0.479 & 0.020 & 0.745 & 0.040 & 0.239 & 0.020 & 0.446 & 0.030 \\
 & & Sexual Orientation & 0.923 & 0.050 & 0.418 & 0.010 & 0.177 & 0.010 & 0.258 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.874 & 0.040 & 0.985 & 0.050 & 0.268 & 0.020 & 0.668 & 0.040 \\
 & & Gender & 0.186 & 0.010 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.010 & 0.745 & 0.040 & 0.732 & 0.050 \\
 & & Immigration Status & 0.719 & 0.030 & 0.544 & 0.030 & 0.576 & 0.030 & 0.501 & 0.020 \\
 & & Race & 0.479 & 0.020 & 0.828 & 0.040 & \cellcolor[HTML]{F4CCCC}0.031 & 0.010 & 0.622 & 0.030 \\
 & & Sexual Orientation & 0.923 & 0.050 & 0.278 & 0.020 & 0.842 & 0.050 & 0.060 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.874 & 0.040 & \cellcolor[HTML]{F4CCCC}0.017 & 0.010 & 0.268 & 0.020 & 0.304 & 0.020 \\
 & & Gender & 0.186 & 0.010 & 0.947 & 0.050 & 0.745 & 0.040 & 0.964 & 0.050 \\
 & & Immigration Status & 0.719 & 0.030 & 0.264 & 0.040 & 0.576 & 0.030 & 0.517 & 0.040 \\
 & & Race & 0.479 & 0.020 & 0.262 & 0.030 & \cellcolor[HTML]{F4CCCC}0.031 & 0.010 & 0.446 & 0.030 \\
 & & Sexual Orientation & 0.923 & 0.050 & \cellcolor[HTML]{F4CCCC}0.036 & 0.020 & 0.842 & 0.050 & 0.258 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.874 & 0.040 & 0.381 & 0.040 & 0.268 & 0.020 & 0.304 & 0.020 \\
 & & Gender & 0.186 & 0.010 & 0.149 & 0.020 & 0.745 & 0.040 & 0.964 & 0.050 \\
 & & Immigration Status & 0.719 & 0.030 & 0.153 & 0.030 & 0.576 & 0.030 & 0.517 & 0.040 \\
 & & Race & 0.479 & 0.020 & 0.583 & 0.050 & \cellcolor[HTML]{F4CCCC}0.031 & 0.010 & 0.446 & 0.030 \\
 & & Sexual Orientation & 0.923 & 0.050 & 0.139 & 0.010 & 0.842 & 0.050 & 0.258 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.874 & 0.040 & \cellcolor[HTML]{F4CCCC}0.017 & 0.010 & 0.268 & 0.020 & 0.304 & 0.020 \\
 & & Gender & 0.186 & 0.010 & 0.947 & 0.050 & 0.745 & 0.040 & 0.964 & 0.050 \\
 & & Immigration Status & 0.719 & 0.030 & 0.264 & 0.040 & 0.576 & 0.030 & 0.517 & 0.040 \\
 & & Race & 0.479 & 0.020 & 0.262 & 0.030 & \cellcolor[HTML]{F4CCCC}0.031 & 0.010 & 0.446 & 0.030 \\
 & & Sexual Orientation & 0.923 & 0.050 & \cellcolor[HTML]{F4CCCC}0.036 & 0.020 & 0.842 & 0.050 & 0.258 & 0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fnr, Xu\_interpretable.}
\label{tab:appendix_fnr_xu_interpretable}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Xu\_personalized \etal \cite{xu2021leveraging} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.417 & 0.040 & 0.633 & 0.050 & 0.604 & 0.040 & 0.239 & 0.020 \\
 & & Gender & 0.654 & 0.050 & 0.494 & 0.040 & \cellcolor[HTML]{F4CCCC}0.027 & 0.010 & 0.361 & 0.030 \\
 & & Immigration Status & 0.187 & 0.020 & 0.387 & 0.020 & 0.195 & 0.030 & 0.927 & 0.050 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.048 & 0.010 & 0.349 & 0.010 & 0.075 & 0.020 & 0.661 & 0.040 \\
 & & Sexual Orientation & 0.281 & 0.030 & 0.434 & 0.030 & 0.743 & 0.050 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.417 & 0.040 & 0.633 & 0.050 & 0.604 & 0.040 & 0.239 & 0.020 \\
 & & Gender & 0.654 & 0.050 & 0.494 & 0.040 & \cellcolor[HTML]{F4CCCC}0.027 & 0.010 & 0.361 & 0.030 \\
 & & Immigration Status & 0.187 & 0.020 & 0.387 & 0.020 & 0.195 & 0.030 & 0.927 & 0.050 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.048 & 0.010 & 0.349 & 0.010 & 0.075 & 0.020 & 0.661 & 0.040 \\
 & & Sexual Orientation & 0.281 & 0.030 & 0.434 & 0.030 & 0.743 & 0.050 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.417 & 0.040 & 0.633 & 0.050 & 0.604 & 0.040 & 0.239 & 0.020 \\
 & & Gender & 0.654 & 0.050 & 0.494 & 0.040 & \cellcolor[HTML]{F4CCCC}0.027 & 0.010 & 0.361 & 0.030 \\
 & & Immigration Status & 0.187 & 0.020 & 0.387 & 0.020 & 0.195 & 0.030 & 0.927 & 0.050 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.048 & 0.010 & 0.349 & 0.010 & 0.075 & 0.020 & 0.661 & 0.040 \\
 & & Sexual Orientation & 0.281 & 0.030 & 0.434 & 0.030 & 0.743 & 0.050 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.417 & 0.040 & 0.633 & 0.050 & 0.604 & 0.040 & 0.239 & 0.020 \\
 & & Gender & 0.654 & 0.050 & 0.494 & 0.040 & \cellcolor[HTML]{F4CCCC}0.027 & 0.010 & 0.361 & 0.030 \\
 & & Immigration Status & 0.187 & 0.020 & 0.387 & 0.020 & 0.195 & 0.030 & 0.927 & 0.050 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.048 & 0.010 & 0.349 & 0.010 & 0.075 & 0.020 & 0.661 & 0.040 \\
 & & Sexual Orientation & 0.281 & 0.030 & 0.434 & 0.030 & 0.743 & 0.050 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.417 & 0.040 & 0.633 & 0.050 & 0.604 & 0.040 & 0.239 & 0.020 \\
 & & Gender & 0.654 & 0.050 & 0.494 & 0.040 & \cellcolor[HTML]{F4CCCC}0.027 & 0.010 & 0.361 & 0.030 \\
 & & Immigration Status & 0.187 & 0.020 & 0.387 & 0.020 & 0.195 & 0.030 & 0.927 & 0.050 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.048 & 0.010 & 0.349 & 0.010 & 0.075 & 0.020 & 0.661 & 0.040 \\
 & & Sexual Orientation & 0.281 & 0.030 & 0.434 & 0.030 & 0.743 & 0.050 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fnr, Xu\_personalized.}
\label{tab:appendix_fnr_xu_personalized}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Canzian \etal \cite{canzian2015trajectories} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.415 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.045 & 0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.288 & 0.030 & 0.077 & 0.020 & 0.230 & 0.030 & 0.549 & 0.030 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 & 0.881 & 0.050 & 0.644 & 0.050 & 0.297 & 0.020 \\
 & & Race & 0.244 & 0.020 & 0.495 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.721 & 0.040 \\
 & & Sexual Orientation & 0.627 & 0.050 & 0.102 & 0.030 & 0.351 & 0.040 & 0.821 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.020 & 0.214 & 0.030 & \cellcolor[HTML]{F4CCCC}0.023 & 0.020 \\
 & & Gender & 1.000 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.146 & 0.020 & \cellcolor[HTML]{F4CCCC}0.031 & 0.030 \\
 & & Immigration Status & 1.000 & 0.030 & 0.861 & 0.050 & 0.347 & 0.040 & 0.706 & 0.050 \\
 & & Race & 1.000 & 0.030 & 0.104 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.062 & 0.040 \\
 & & Sexual Orientation & 1.000 & 0.030 & 0.414 & 0.040 & 0.440 & 0.050 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.332 & 0.040 & 0.259 & 0.040 & 0.067 & 0.020 & 0.802 & 0.050 \\
 & & Gender & 0.751 & 0.050 & 0.709 & 0.050 & 0.708 & 0.030 & 0.260 & 0.020 \\
 & & Immigration Status & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.983 & 0.050 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.035 & 0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.621 & 0.040 \\
 & & Sexual Orientation & 0.066 & 0.030 & 0.172 & 0.030 & 0.795 & 0.040 & 0.427 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 1.000 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.190 & 0.020 & \cellcolor[HTML]{F4CCCC}0.023 & 0.020 \\
 & & Gender & 1.000 & 0.030 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & 0.769 & 0.040 & \cellcolor[HTML]{F4CCCC}0.031 & 0.030 \\
 & & Immigration Status & 1.000 & 0.030 & 0.867 & 0.040 & 0.745 & 0.030 & 0.553 & 0.050 \\
 & & Race & 1.000 & 0.030 & 0.219 & 0.030 & \cellcolor[HTML]{F4CCCC}0.018 & 0.010 & 0.062 & 0.040 \\
 & & Sexual Orientation & 1.000 & 0.030 & 0.878 & 0.050 & 0.984 & 0.050 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.150 & 0.020 & \cellcolor[HTML]{F4CCCC}0.022 & 0.010 & 0.175 & 0.020 & 0.289 & 0.040 \\
 & & Gender & 0.883 & 0.050 & 0.362 & 0.020 & 0.907 & 0.050 & 0.137 & 0.030 \\
 & & Immigration Status & 0.353 & 0.040 & 0.666 & 0.040 & 0.295 & 0.030 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Race & 0.190 & 0.030 & 0.642 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.967 & 0.050 \\
 & & Sexual Orientation & 0.077 & 0.010 & 0.750 & 0.050 & 0.523 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fpr, Canzian.}
\label{tab:appendix_fpr_canzian}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Saeb \etal \cite{saeb2015mobile} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.381 & 0.040 & \cellcolor[HTML]{F4CCCC}0.033 & 0.030 & 0.210 & 0.020 & 0.910 & 0.050 \\
 & & Immigration Status & 0.477 & 0.050 & 0.790 & 0.040 & 0.835 & 0.050 & 0.103 & 0.040 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.012 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.020 & 0.590 & 0.030 & 0.052 & 0.030 \\
 & & Sexual Orientation & \cellcolor[HTML]{F4CCCC}0.036 & 0.030 & 0.892 & 0.050 & 0.723 & 0.040 & \cellcolor[HTML]{F4CCCC}0.040 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.080 & 0.020 & 0.903 & 0.050 & 0.636 & 0.050 \\
 & & Gender & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.061 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.133 & 0.050 & 0.491 & 0.050 & 0.054 & 0.020 & \cellcolor[HTML]{F4CCCC}0.022 & \cellcolor[HTML]{F4CCCC}0.030 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.018 & \cellcolor[HTML]{F4CCCC}0.030 & 0.445 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Sexual Orientation & \cellcolor[HTML]{F4CCCC}0.029 & \cellcolor[HTML]{F4CCCC}0.040 & 0.089 & 0.030 & 0.341 & 0.040 & 0.552 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.020 & 0.395 & 0.030 & 0.587 & 0.050 & 0.187 & 0.020 \\
 & & Gender & 0.644 & 0.050 & 0.396 & 0.040 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.020 & 0.549 & 0.050 \\
 & & Immigration Status & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.081 & 0.030 & 0.469 & 0.040 \\
 & & Race & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.030 & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Sexual Orientation & \cellcolor[HTML]{F4CCCC}0.036 & \cellcolor[HTML]{F4CCCC}0.040 & 0.609 & 0.050 & 0.094 & 0.040 & 0.266 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.020 & 1.000 & 0.030 & 0.793 & 0.050 & 0.425 & 0.040 \\
 & & Gender & 0.511 & 0.050 & 1.000 & 0.030 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.273 & 0.030 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.030 & 1.000 & 0.030 & 0.052 & 0.020 & 0.098 & 0.020 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 1.000 & 0.030 & 0.247 & 0.030 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Sexual Orientation & 0.294 & 0.040 & 1.000 & 0.030 & 0.339 & 0.040 & 0.578 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.269 & 0.020 & 1.000 & 0.030 & 0.984 & 0.050 & 0.672 & 0.040 \\
 & & Gender & 0.644 & 0.050 & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}0.026 & 0.020 & 0.281 & 0.030 \\
 & & Immigration Status & 0.222 & 0.010 & 1.000 & 0.030 & 0.099 & 0.030 & 0.840 & 0.050 \\
 & & Race & 0.629 & 0.040 & 1.000 & 0.030 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 & 0.133 & 0.020 \\
 & & Sexual Orientation & 0.279 & 0.030 & 1.000 & 0.030 & 0.823 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fpr, Saeb.}
\label{tab:appendix_fpr_saeb}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Farhan \etal \cite{farhan2016behavior} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 & 0.125 & 0.020 & 0.103 & 0.010 & 0.394 & 0.040 \\
 & & Gender & 0.537 & 0.040 & \cellcolor[HTML]{F4CCCC}0.023 & 0.010 & 0.131 & 0.020 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.601 & 0.050 & 0.367 & 0.030 & 0.480 & 0.040 & 0.327 & 0.030 \\
 & & Race & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.020 & 0.538 & 0.040 & 0.204 & 0.030 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Sexual Orientation & \cellcolor[HTML]{EA9999}0.010 & \cellcolor[HTML]{F4CCCC}0.030 & 0.550 & 0.050 & 0.985 & 0.050 & 0.847 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.549 & 0.030 & 0.855 & 0.050 & 0.744 & 0.050 & 0.512 & 0.050 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.015 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.570 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.104 & 0.020 & 0.636 & 0.040 & 0.315 & 0.030 & 0.298 & 0.040 \\
 & & Race & 0.609 & 0.040 & 0.359 & 0.020 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Sexual Orientation & 0.670 & 0.050 & 0.452 & 0.030 & 0.144 & 0.020 & 0.207 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.650 & 0.050 & 0.146 & 0.020 & 0.112 & 0.030 & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 \\
 & & Gender & 0.580 & 0.030 & 0.236 & 0.040 & 0.087 & 0.010 & \cellcolor[HTML]{F4CCCC}0.048 & 0.030 \\
 & & Immigration Status & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.016 & 0.010 & 0.159 & 0.040 & 0.105 & 0.040 \\
 & & Race & 0.647 & 0.040 & 0.354 & 0.050 & 0.088 & 0.020 & \cellcolor[HTML]{F4CCCC}0.022 & 0.020 \\
 & & Sexual Orientation & 0.173 & 0.020 & 0.154 & 0.030 & 0.292 & 0.050 & 0.323 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.197 & 0.030 & 0.668 & 0.040 & 0.183 & 0.030 & 0.500 & 0.040 \\
 & & Gender & 0.970 & 0.050 & 0.088 & 0.020 & 0.975 & 0.050 & 0.833 & 0.050 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.010 & 0.010 & 0.061 & 0.010 & 0.825 & 0.040 & \cellcolor[HTML]{F4CCCC}0.035 & 0.010 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.030 & 0.020 & 0.272 & 0.030 & \cellcolor[HTML]{F4CCCC}0.022 & 0.010 & 0.244 & 0.030 \\
 & & Sexual Orientation & 0.251 & 0.040 & 0.701 & 0.050 & 0.057 & 0.020 & 0.079 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.483 & 0.010 & 0.581 & 0.040 & 0.887 & 0.050 & 0.222 & 0.050 \\
 & & Gender & 0.725 & 0.050 & 0.088 & 0.010 & 0.298 & 0.030 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.600 & 0.030 & 0.127 & 0.020 & 0.539 & 0.040 & 0.145 & 0.040 \\
 & & Race & 0.656 & 0.040 & 0.417 & 0.030 & 0.165 & 0.010 & 0.065 & 0.030 \\
 & & Sexual Orientation & 0.593 & 0.020 & 0.916 & 0.050 & 0.168 & 0.020 & \cellcolor[HTML]{F4CCCC}0.038 & 0.020 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fpr, Farhan.}
\label{tab:appendix_fpr_farhan}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Wahle \etal \cite{wahle2016mobile} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.450 & 0.030 & 0.102 & 0.030 & 0.222 & 0.020 & 0.089 & 0.040 \\
 & & Immigration Status & 0.821 & 0.040 & 0.838 & 0.050 & 0.798 & 0.040 & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Race & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.010 & 0.057 & 0.020 & 0.280 & 0.030 & \cellcolor[HTML]{F4CCCC}0.045 & 0.030 \\
 & & Sexual Orientation & 0.990 & 0.050 & 0.282 & 0.040 & 0.998 & 0.050 & 0.186 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.020 & 0.010 & 0.259 & 0.020 & 0.656 & 0.050 & 0.894 & 0.040 \\
 & & Gender & 0.958 & 0.050 & 0.123 & 0.010 & 0.099 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.783 & 0.030 & 0.753 & 0.040 & 0.121 & 0.020 & 0.519 & 0.020 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.020 & 0.020 & 0.868 & 0.050 & 0.640 & 0.040 & 0.956 & 0.050 \\
 & & Sexual Orientation & 0.949 & 0.040 & 0.753 & 0.030 & 0.395 & 0.030 & 0.820 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.031 & 0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & 0.273 & 0.020 & 0.139 & 0.040 \\
 & & Gender & 0.334 & 0.030 & 0.459 & 0.040 & 0.344 & 0.030 & 0.934 & 0.050 \\
 & & Immigration Status & 0.912 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.066 & 0.010 & 0.095 & 0.020 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & 0.137 & 0.030 & 0.551 & 0.040 & 0.065 & 0.010 \\
 & & Sexual Orientation & 0.918 & 0.050 & 0.951 & 0.050 & 0.990 & 0.050 & 0.099 & 0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & 0.831 & 0.040 & 0.382 & 0.040 \\
 & & Gender & 0.450 & 0.040 & 0.459 & 0.030 & 0.280 & 0.010 & 0.879 & 0.050 \\
 & & Immigration Status & 0.821 & 0.050 & 0.783 & 0.040 & 0.357 & 0.020 & 0.285 & 0.030 \\
 & & Race & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.229 & 0.020 & 0.538 & 0.030 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Sexual Orientation & 0.441 & 0.030 & 0.951 & 0.050 & 0.943 & 0.050 & 0.112 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.011 & \cellcolor[HTML]{F4CCCC}0.020 & 0.137 & 0.010 & 0.697 & 0.030 & 0.071 & 0.020 \\
 & & Gender & 0.450 & 0.030 & 0.337 & 0.020 & 0.768 & 0.040 & 0.985 & 0.050 \\
 & & Immigration Status & 0.821 & 0.040 & 0.442 & 0.030 & 0.273 & 0.020 & 0.458 & 0.030 \\
 & & Race & \cellcolor[HTML]{EA9999}0.007 & \cellcolor[HTML]{F4CCCC}0.010 & 0.742 & 0.050 & 0.199 & 0.010 & 0.833 & 0.040 \\
 & & Sexual Orientation & 0.990 & 0.050 & 0.507 & 0.040 & 0.990 & 0.050 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fpr, Wahle.}
\label{tab:appendix_fpr_wahle}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Lu \etal \cite{lu2018joint} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.183 & 0.030 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.429 & 0.030 & 0.829 & 0.050 & 0.975 & 0.050 & \cellcolor[HTML]{F4CCCC}0.012 & \cellcolor[HTML]{F4CCCC}0.020 \\
 & & Immigration Status & 0.890 & 0.050 & 0.099 & 0.030 & \cellcolor[HTML]{F4CCCC}0.041 & 0.020 & 0.111 & 0.040 \\
 & & Race & 0.836 & 0.040 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.020 & 0.360 & 0.040 & 0.720 & 0.050 \\
 & & Sexual Orientation & 0.146 & 0.020 & 0.319 & 0.040 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{F4CCCC}0.016 & \cellcolor[HTML]{F4CCCC}0.030 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.459 & 0.040 & 0.391 & 0.040 & 0.478 & 0.050 & 0.706 & 0.030 \\
 & & Gender & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.060 & 0.030 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & 0.482 & 0.050 & 0.425 & 0.050 & 0.471 & 0.040 & 0.235 & 0.020 \\
 & & Race & 0.285 & 0.030 & 0.116 & 0.020 & \cellcolor[HTML]{F4CCCC}0.017 & 0.010 & 0.961 & 0.050 \\
 & & Sexual Orientation & 0.147 & 0.020 & 0.371 & 0.030 & \cellcolor[HTML]{F4CCCC}0.030 & 0.020 & 0.857 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.020 & 0.477 & 0.050 & \cellcolor[HTML]{F4CCCC}0.016 & 0.010 & 0.262 & 0.020 \\
 & & Gender & 0.996 & 0.050 & 0.436 & 0.040 & 0.140 & 0.040 & 0.604 & 0.050 \\
 & & Immigration Status & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.072 & 0.030 & 0.111 & 0.010 \\
 & & Race & 0.771 & 0.030 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}0.020 & 0.060 & 0.020 & 0.504 & 0.030 \\
 & & Sexual Orientation & 0.779 & 0.040 & 0.093 & 0.030 & 0.202 & 0.050 & 0.579 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.020 & 0.940 & 0.050 & 0.541 & 0.030 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & 0.958 & 0.050 & 0.059 & 0.030 & 0.961 & 0.050 & 0.088 & 0.030 \\
 & & Immigration Status & 0.064 & 0.030 & \cellcolor[HTML]{EA9999}0.002 & \cellcolor[HTML]{F4CCCC}0.020 & \cellcolor[HTML]{F4CCCC}0.049 & 0.020 & \cellcolor[HTML]{F4CCCC}0.041 & 0.020 \\
 & & Race & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 0.727 & 0.040 & 0.199 & 0.040 \\
 & & Sexual Orientation & 0.433 & 0.040 & 0.089 & 0.040 & \cellcolor[HTML]{F4CCCC}0.040 & 0.010 & 0.543 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.954 & 0.050 & 0.176 & 0.020 & 0.206 & 0.020 & 0.231 & 0.050 \\
 & & Gender & 0.087 & 0.030 & 0.064 & 0.010 & 0.771 & 0.050 & 0.187 & 0.030 \\
 & & Immigration Status & 0.090 & 0.040 & 0.430 & 0.040 & 0.198 & 0.010 & \cellcolor[HTML]{EA9999}0.006 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Race & 0.073 & 0.020 & 0.530 & 0.050 & 0.208 & 0.030 & 0.230 & 0.040 \\
 & & Sexual Orientation & \cellcolor[HTML]{EA9999}0.001 & \cellcolor[HTML]{F4CCCC}0.010 & 0.264 & 0.030 & 0.531 & 0.040 & \cellcolor[HTML]{F4CCCC}0.033 & 0.020 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fpr, Lu.}
\label{tab:appendix_fpr_lu}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Wang \etal \cite{wang2018tracking} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.024 & 0.020 & 1.000 & 0.030 & 0.129 & 0.040 & 0.121 & 0.040 \\
 & & Immigration Status & 0.612 & 0.030 & 1.000 & 0.030 & 0.373 & 0.050 & 0.101 & 0.030 \\
 & & Race & 0.994 & 0.050 & 1.000 & 0.030 & 0.121 & 0.030 & \cellcolor[HTML]{F4CCCC}0.023 & 0.020 \\
 & & Sexual Orientation & 0.985 & 0.040 & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}0.030 & 0.020 & 0.450 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.641 & 0.050 & 1.000 & 0.030 & 0.410 & 0.050 & 0.552 & 0.050 \\
 & & Gender & 0.440 & 0.030 & 1.000 & 0.030 & 0.129 & 0.020 & 0.418 & 0.030 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & 1.000 & 0.030 & 0.143 & 0.030 & 0.071 & 0.020 \\
 & & Race & 0.582 & 0.040 & 1.000 & 0.030 & 0.308 & 0.040 & 0.543 & 0.040 \\
 & & Sexual Orientation & 0.343 & 0.020 & 1.000 & 0.030 & 0.125 & 0.010 & \cellcolor[HTML]{F4CCCC}0.028 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & \cellcolor[HTML]{F4CCCC}0.049 & 0.010 & 0.437 & 0.020 & 0.410 & 0.050 & 0.736 & 0.050 \\
 & & Gender & 0.244 & 0.020 & 0.857 & 0.050 & 0.129 & 0.020 & 0.623 & 0.040 \\
 & & Immigration Status & 0.498 & 0.040 & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 & 0.143 & 0.030 & 0.364 & 0.030 \\
 & & Race & 0.369 & 0.030 & 0.737 & 0.040 & 0.308 & 0.040 & 0.186 & 0.020 \\
 & & Sexual Orientation & 0.782 & 0.050 & 0.670 & 0.030 & 0.125 & 0.010 & \cellcolor[HTML]{EA9999}0.004 & \cellcolor[HTML]{F4CCCC}0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & \cellcolor[HTML]{EA9999}0.005 & \cellcolor[HTML]{F4CCCC}0.010 & 1.000 & 0.030 & 0.610 & 0.050 & 0.552 & 0.050 \\
 & & Gender & \cellcolor[HTML]{EA9999}0.008 & \cellcolor[HTML]{F4CCCC}0.020 & 1.000 & 0.030 & 0.306 & 0.040 & 0.418 & 0.030 \\
 & & Immigration Status & 0.466 & 0.040 & 1.000 & 0.030 & 0.094 & 0.010 & 0.071 & 0.020 \\
 & & Race & \cellcolor[HTML]{F4CCCC}0.024 & \cellcolor[HTML]{F4CCCC}0.030 & 1.000 & 0.030 & 0.191 & 0.020 & 0.543 & 0.040 \\
 & & Sexual Orientation & 0.611 & 0.050 & 1.000 & 0.030 & 0.276 & 0.030 & \cellcolor[HTML]{F4CCCC}0.028 & 0.010 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.069 & 0.030 & 1.000 & 0.030 & 0.507 & 0.050 & 0.552 & 0.050 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.028 & 0.010 & 1.000 & 0.030 & 0.206 & 0.030 & 0.418 & 0.030 \\
 & & Immigration Status & 0.067 & 0.020 & 1.000 & 0.030 & 0.116 & 0.020 & 0.071 & 0.020 \\
 & & Race & 0.424 & 0.050 & 1.000 & 0.030 & 0.244 & 0.040 & 0.543 & 0.040 \\
 & & Sexual Orientation & 0.392 & 0.040 & 1.000 & 0.030 & 0.106 & 0.010 & \cellcolor[HTML]{F4CCCC}0.028 & 0.010 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fpr, Wang.}
\label{tab:appendix_fpr_wang}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Xu\_interpretable \etal \cite{xu2019leveraging} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.189 & 0.030 & \cellcolor[HTML]{F4CCCC}0.024 & 0.020 & 0.432 & 0.040 & 0.395 & 0.030 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & \cellcolor[HTML]{F4CCCC}0.019 & 0.010 & 0.233 & 0.020 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.023 & 0.020 & 0.494 & 0.040 & 0.769 & 0.050 & 0.907 & 0.050 \\
 & & Race & 0.366 & 0.050 & 0.084 & 0.030 & 0.222 & 0.010 & 0.388 & 0.020 \\
 & & Sexual Orientation & 0.195 & 0.040 & 0.518 & 0.050 & 0.406 & 0.030 & 0.441 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.189 & 0.030 & 0.430 & 0.020 & 0.613 & 0.040 & 0.642 & 0.040 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & 0.487 & 0.030 & \cellcolor[HTML]{F4CCCC}0.038 & 0.010 & \cellcolor[HTML]{F4CCCC}0.045 & 0.010 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.023 & 0.020 & 0.704 & 0.040 & 0.651 & 0.050 & 0.846 & 0.050 \\
 & & Race & 0.366 & 0.050 & 0.116 & 0.010 & 0.569 & 0.030 & 0.605 & 0.030 \\
 & & Sexual Orientation & 0.195 & 0.040 & 0.748 & 0.050 & 0.132 & 0.020 & 0.285 & 0.020 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.189 & 0.030 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 & 0.613 & 0.040 & 0.395 & 0.030 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & 0.148 & 0.030 & \cellcolor[HTML]{F4CCCC}0.038 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.023 & 0.020 & 0.080 & 0.020 & 0.651 & 0.050 & 0.907 & 0.050 \\
 & & Race & 0.366 & 0.050 & 0.450 & 0.050 & 0.569 & 0.030 & 0.388 & 0.020 \\
 & & Sexual Orientation & 0.195 & 0.040 & 0.449 & 0.040 & 0.132 & 0.020 & 0.441 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.189 & 0.030 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 & 0.613 & 0.040 & 0.395 & 0.030 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & 0.256 & 0.030 & \cellcolor[HTML]{F4CCCC}0.038 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.023 & 0.020 & 0.511 & 0.040 & 0.651 & 0.050 & 0.907 & 0.050 \\
 & & Race & 0.366 & 0.050 & 0.116 & 0.020 & 0.569 & 0.030 & 0.388 & 0.020 \\
 & & Sexual Orientation & 0.195 & 0.040 & 0.841 & 0.050 & 0.132 & 0.020 & 0.441 & 0.040 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.189 & 0.030 & \cellcolor[HTML]{EA9999}0.003 & \cellcolor[HTML]{F4CCCC}0.010 & 0.613 & 0.040 & 0.395 & 0.030 \\
 & & Gender & \cellcolor[HTML]{F4CCCC}0.011 & 0.010 & 0.148 & 0.030 & \cellcolor[HTML]{F4CCCC}0.038 & 0.010 & \cellcolor[HTML]{E06666}0.000 & \cellcolor[HTML]{F4CCCC}0.010 \\
 & & Immigration Status & \cellcolor[HTML]{F4CCCC}0.023 & 0.020 & 0.080 & 0.020 & 0.651 & 0.050 & 0.907 & 0.050 \\
 & & Race & 0.366 & 0.050 & 0.450 & 0.050 & 0.569 & 0.030 & 0.388 & 0.020 \\
 & & Sexual Orientation & 0.195 & 0.040 & 0.449 & 0.040 & 0.132 & 0.020 & 0.441 & 0.040 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fpr, Xu\_interpretable.}
\label{tab:appendix_fpr_xu_interpretable}
\end{table}
 
 
 
 
 
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{|l|l|l|rr|rr|rr|rr|}\hline
&&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\textbf{Added Sub-attributes}} & \multirow{-2}{*}{\textbf{Sensitive Sub-attributes}} & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  & \multicolumn{1}{c}{p values}  & \multicolumn{1}{c|}{q values}  \\\hline
 
 \multirow{25}{*}{Xu\_personalized \etal \cite{xu2021leveraging} }& \multirow{5}{*}{First-gen College Student} & First-gen College Student & 0.300 & 0.020 & 0.819 & 0.040 & 0.609 & 0.020 & 0.178 & 0.010 \\
 & & Gender & 0.751 & 0.040 & 0.959 & 0.050 & 0.069 & 0.010 & 0.182 & 0.020 \\
 & & Immigration Status & 0.775 & 0.050 & 0.176 & 0.020 & 0.609 & 0.020 & 0.342 & 0.030 \\
 & & Race & 0.436 & 0.030 & \cellcolor[HTML]{F4CCCC}0.022 & 0.010 & 0.881 & 0.050 & 0.682 & 0.040 \\
 & & Sexual Orientation & 0.254 & 0.010 & 0.627 & 0.030 & 0.833 & 0.040 & 0.723 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Gender} & First-gen College Student & 0.300 & 0.020 & 0.819 & 0.040 & 0.609 & 0.020 & 0.178 & 0.010 \\
 & & Gender & 0.751 & 0.040 & 0.959 & 0.050 & 0.069 & 0.010 & 0.182 & 0.020 \\
 & & Immigration Status & 0.775 & 0.050 & 0.176 & 0.020 & 0.609 & 0.020 & 0.342 & 0.030 \\
 & & Race & 0.436 & 0.030 & \cellcolor[HTML]{F4CCCC}0.022 & 0.010 & 0.881 & 0.050 & 0.682 & 0.040 \\
 & & Sexual Orientation & 0.254 & 0.010 & 0.627 & 0.030 & 0.833 & 0.040 & 0.723 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Immigration Status} & First-gen College Student & 0.300 & 0.020 & 0.819 & 0.040 & 0.609 & 0.020 & 0.178 & 0.010 \\
 & & Gender & 0.751 & 0.040 & 0.959 & 0.050 & 0.069 & 0.010 & 0.182 & 0.020 \\
 & & Immigration Status & 0.775 & 0.050 & 0.176 & 0.020 & 0.609 & 0.020 & 0.342 & 0.030 \\
 & & Race & 0.436 & 0.030 & \cellcolor[HTML]{F4CCCC}0.022 & 0.010 & 0.881 & 0.050 & 0.682 & 0.040 \\
 & & Sexual Orientation & 0.254 & 0.010 & 0.627 & 0.030 & 0.833 & 0.040 & 0.723 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Race} & First-gen College Student & 0.300 & 0.020 & 0.819 & 0.040 & 0.609 & 0.020 & 0.178 & 0.010 \\
 & & Gender & 0.751 & 0.040 & 0.959 & 0.050 & 0.069 & 0.010 & 0.182 & 0.020 \\
 & & Immigration Status & 0.775 & 0.050 & 0.176 & 0.020 & 0.609 & 0.020 & 0.342 & 0.030 \\
 & & Race & 0.436 & 0.030 & \cellcolor[HTML]{F4CCCC}0.022 & 0.010 & 0.881 & 0.050 & 0.682 & 0.040 \\
 & & Sexual Orientation & 0.254 & 0.010 & 0.627 & 0.030 & 0.833 & 0.040 & 0.723 & 0.050 \\
\cline{2-11}
 & \multirow{5}{*}{Sexual Orientation} & First-gen College Student & 0.300 & 0.020 & 0.819 & 0.040 & 0.609 & 0.020 & 0.178 & 0.010 \\
 & & Gender & 0.751 & 0.040 & 0.959 & 0.050 & 0.069 & 0.010 & 0.182 & 0.020 \\
 & & Immigration Status & 0.775 & 0.050 & 0.176 & 0.020 & 0.609 & 0.020 & 0.342 & 0.030 \\
 & & Race & 0.436 & 0.030 & \cellcolor[HTML]{F4CCCC}0.022 & 0.010 & 0.881 & 0.050 & 0.682 & 0.040 \\
 & & Sexual Orientation & 0.254 & 0.010 & 0.627 & 0.030 & 0.833 & 0.040 & 0.723 & 0.050 \\
\cline{2-11}
\hline
 
\end{tabular}}
\caption{Fpr, Xu\_personalized.}
\label{tab:appendix_fpr_xu_personalized}
\end{table}
 
 
 
 
 


==> fig_tab_alg/tab_fnr_w_t_demo.tex <==
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\caption{Algorithmic fairness evaluation results through the \textbf{disparity in false negative rate} (without incorporating demographic data into the training and testing process). The p-value serves as a significance threshold, indicating the likelihood that the observed data could have occurred by random chance before applying the Benjamini-Hochberg correction, while the q-value is the adjusted p-value by Benjamini-Hochberg correction. Significance is marked *$<0.05$, **$<0.01$, ***$<0.001$. Our analyses and conclusions are based on q-values.}
\resizebox{0.9\textwidth}{!}{\begin{tabular}{|l|l|rr|rr|rr|rr|}\hline
&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\\cline{3-10}
\multirow{-2}{*}{\textbf{Algorithms}} &\multirow{-2}{*}{\textbf{Sensitive Attributes}} & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  \\\hline
  
 \multirow{5}{*}{Wahle \etal \cite{wahle2016mobile}} & First-gen College Student & 1.000 & 0.030 & 0.423 & 0.050 & 0.576 & 0.030 & 0.565 & 0.050 \\
  & Gender & 1.000 & 0.030 & 0.155 & 0.030 & 0.181 & 0.010 & 0.470 & 0.030 \\
  & Immigration Status & 1.000 & 0.030 & 0.350 & 0.040 & 0.562 & 0.020 & 0.080 & 0.010 \\
  & Race & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.037 & 0.010 & 0.805 & 0.050 & 0.328 & 0.020 \\
  & Sexual Orientation & 1.000 & 0.030 & 0.147 & 0.020 & 0.687 & 0.040 & 0.494 & 0.040 \\
\hline
 
 \multirow{5}{*}{Saeb \etal \cite{saeb2015mobile}} & First-gen College Student & 0.069 & 0.030 & 1.000 & 0.030 & 0.870 & 0.050 & 0.119 & 0.030 \\
  & Gender & 0.315 & 0.040 & 1.000 & 0.030 & 0.452 & 0.030 & 0.416 & 0.040 \\
  & Immigration Status & \cellcolor[HTML]{EA9999}**0.006 & \cellcolor[HTML]{F4CCCC}*0.010 & 1.000 & 0.030 & 0.550 & 0.040 & 1.000 & 0.050 \\
  & Race & 0.378 & 0.050 & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.041 & 0.010 & 0.060 & 0.020 \\
  & Sexual Orientation & \cellcolor[HTML]{F4CCCC}*0.016 & \cellcolor[HTML]{F4CCCC}*0.020 & 1.000 & 0.030 & 0.266 & 0.020 & \cellcolor[HTML]{EA9999}**0.004 & \cellcolor[HTML]{F4CCCC}*0.010 \\
\hline
 
 \multirow{5}{*}{Farhan \etal \cite{farhan2016behavior}} & First-gen College Student & 0.302 & 0.020 & 0.386 & 0.030 & 0.519 & 0.040 & \cellcolor[HTML]{F4CCCC}*0.025 & 0.010 \\
  & Gender & 0.369 & 0.030 & 0.111 & 0.020 & 0.503 & 0.030 & 0.601 & 0.040 \\
  & Immigration Status & 0.752 & 0.040 & \cellcolor[HTML]{EA9999}**0.003 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.223 & 0.010 & 0.704 & 0.050 \\
  & Race & 0.861 & 0.050 & 0.858 & 0.050 & 0.307 & 0.020 & 0.141 & 0.020 \\
  & Sexual Orientation & 0.083 & 0.010 & 0.470 & 0.040 & 0.728 & 0.050 & 0.408 & 0.030 \\
\hline

\multirow{5}{*}{Canzian \etal \cite{canzian2015trajectories}} & First-gen College Student & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.016 & 0.010 & 0.173 & 0.020 & 0.070 & 0.030 \\
  & Gender & 1.000 & 0.030 & 0.200 & 0.020 & 0.731 & 0.030 & 0.068 & 0.020 \\
  & Immigration Status & 1.000 & 0.030 & 0.949 & 0.050 & 0.769 & 0.040 & 0.614 & 0.040 \\
  & Race & 1.000 & 0.030 & 0.590 & 0.030 & 0.819 & 0.050 & \cellcolor[HTML]{F4CCCC}*0.024 & 0.010 \\
  & Sexual Orientation & 1.000 & 0.030 & 0.898 & 0.040 & 0.108 & 0.010 & 0.847 & 0.050 \\
\hline
 
 \multirow{5}{*}{Wang \etal \cite{wang2018tracking}} & First-gen College Student & 0.928 & 0.050 & 1.000 & 0.030 & 0.312 & 0.030 & 0.577 & 0.040 \\
  & Gender & 0.647 & 0.040 & 1.000 & 0.030 & 0.692 & 0.040 & 0.213 & 0.020 \\
  & Immigration Status & 0.302 & 0.020 & 1.000 & 0.030 & 0.216 & 0.010 & 0.177 & 0.010 \\
  & Race & 0.059 & 0.010 & 1.000 & 0.030 & 0.310 & 0.020 & 0.428 & 0.030 \\
  & Sexual Orientation & 0.403 & 0.030 & 1.000 & 0.030 & 0.892 & 0.050 & 0.650 & 0.050 \\
\hline

 \multirow{5}{*}{Lu \etal \cite{lu2018joint}} & First-gen College Student & \cellcolor[HTML]{EA9999}**0.004 & \cellcolor[HTML]{F4CCCC}*0.020 & \cellcolor[HTML]{F4CCCC}*0.020 & 0.010 & 0.535 & 0.040 & 0.634 & 0.040 \\
  & Gender & 0.843 & 0.030 & 0.529 & 0.020 & 0.535 & 0.040 & 0.253 & 0.030 \\
  & Immigration Status & 0.946 & 0.050 & 0.603 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.050 & 0.010 & 0.920 & 0.050 \\
  & Race & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.679 & 0.040 & 0.186 & 0.020 & 0.064 & 0.010 \\
  & Sexual Orientation & 0.916 & 0.040 & 0.704 & 0.050 & 0.260 & 0.030 & 0.160 & 0.020 \\
\hline
 
 \multirow{5}{*}{Xu\_interpretable \etal \cite{xu2019leveraging}} & First-gen College Student & 0.140 & 0.020 & 0.482 & 0.030 & \cellcolor[HTML]{EA9999}**0.004 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.051 & 0.010 \\
  & Gender & 0.603 & 0.040 & \cellcolor[HTML]{F4CCCC}*0.011 & 0.010 & 0.284 & 0.030 & 0.953 & 0.050 \\
  & Immigration Status & 0.081 & 0.010 & 0.779 & 0.050 & 0.217 & 0.020 & 0.561 & 0.030 \\
  & Race & 0.252 & 0.030 & 0.294 & 0.020 & 0.736 & 0.040 & 0.146 & 0.020 \\
  & Sexual Orientation & 0.805 & 0.050 & 0.723 & 0.040 & 0.978 & 0.050 & 0.930 & 0.040 \\
\hline
 
 \multirow{5}{*}{Xu\_personalized \etal \cite{xu2021leveraging}} & First-gen College Student & 0.335 & 0.040 & 0.400 & 0.030 & 0.604 & 0.040 & 0.239 & 0.020 \\
  & Gender & 0.912 & 0.050 & 0.866 & 0.050 & \cellcolor[HTML]{F4CCCC}*0.027 & 0.010 & 0.361 & 0.030 \\
  & Immigration Status & 0.149 & 0.020 & 0.831 & 0.040 & 0.195 & 0.030 & 0.927 & 0.050 \\
  & Race & 0.060 & 0.010 & 0.316 & 0.020 & 0.075 & 0.020 & 0.661 & 0.040 \\
  & Sexual Orientation & 0.320 & 0.030 & 0.122 & 0.010 & 0.743 & 0.050 & \cellcolor[HTML]{EA9999}**0.005 & \cellcolor[HTML]{F4CCCC}*0.010 \\
\hline
 
 % \multirow{5}{*}{Chikersal \etal \cite{chikersal2021detecting}} & First-gen College Student & 0.727 & 0.030 & 0.965 & 0.050 & 0.991 & 0.050 & 0.081 & 0.020 \\
 %  & Gender & 0.745 & 0.040 & 0.426 & 0.040 & 0.682 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.019 & 0.010 \\
 %  & Immigration Status & 0.872 & 0.050 & 0.288 & 0.030 & 0.095 & 0.010 & 0.509 & 0.040 \\
 %  & Race & 0.628 & 0.020 & \cellcolor[HTML]{F4CCCC}*0.016 & 0.010 & 0.140 & 0.020 & 0.486 & 0.030 \\
 %  & Sexual Orientation & \cellcolor[HTML]{EA9999}**0.002 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.169 & 0.020 & 0.978 & 0.040 & 0.598 & 0.050 \\\hline
\end{tabular}}
\label{tab_fnr_w_t_demo}
\end{table}

==> fig_tab_alg/tab_fpr_w_t_demo.tex <==
\begin{table}[htb!]
\renewcommand{\arraystretch}{1.02}
\caption{Algorithmic fairness evaluation results through the \textbf{disparity in false positive rate} (without incorporating demographic data into the training and testing process). The p-value serves as a significance threshold, indicating the likelihood that the observed data could have occurred by random chance before applying the Benjamini-Hochberg correction, while the q-value is the adjusted p-value by Benjamini-Hochberg correction. Significance is marked *$<0.05$, **$<0.01$, ***$<0.001$. Our analyses and conclusions are based on q-values.}
\resizebox{0.9\textwidth}{!}{\begin{tabular}{|l|l|rr|rr|rr|rr|}\hline
&&
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS1 (2018)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS2 (2019)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS3 (2020)}} &
\multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{DS4 (2021)}} \\\cline{3-10}
\multirow{-2}{*}{\textbf{Algorithms}} &\multirow{-2}{*}{\textbf{Sensitive Attributes}} & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  & \multicolumn{1}{c}{p value}  & \multicolumn{1}{c|}{q value}  \\\hline
 
 \multirow{5}{*}{Wahle \etal \cite{wahle2016mobile}} & First-gen College Student & 1.000 & 0.030 & \cellcolor[HTML]{EA9999}**0.003 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.726 & 0.040 & \cellcolor[HTML]{F4CCCC}*0.037 & 0.020 \\
  & Gender & 1.000 & 0.030 & 0.066 & 0.030 & 0.481 & 0.020 & 0.972 & 0.050 \\
  & Immigration Status & 1.000 & 0.030 & 0.893 & 0.050 & 0.726 & 0.040 & \cellcolor[HTML]{F4CCCC}*0.045 & 0.030 \\
  & Race & 1.000 & 0.030 & 0.063 & 0.020 & 0.622 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.030 & 0.010 \\
  & Sexual Orientation & 1.000 & 0.030 & 0.260 & 0.040 & 0.243 & 0.010 & 0.546 & 0.040 \\
\hline
 
 \multirow{5}{*}{Saeb \etal \cite{saeb2015mobile}} & First-gen College Student & \cellcolor[HTML]{F4CCCC}*0.032 & 0.010 & 1.000 & 0.030 & 0.973 & 0.050 & 0.672 & 0.050 \\
  & Gender & 0.260 & 0.050 & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.014 & \cellcolor[HTML]{F4CCCC}*0.020 & 0.348 & 0.030 \\
  & Immigration Status & 0.089 & 0.040 & 1.000 & 0.030 & 0.206 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.028 & 0.020 \\
  & Race & \cellcolor[HTML]{F4CCCC}*0.050 & 0.020 & 1.000 & 0.030 & \cellcolor[HTML]{EA9999}**0.002 & \cellcolor[HTML]{F4CCCC}*0.010 & \cellcolor[HTML]{F4CCCC}*0.015 & 0.010 \\
  & Sexual Orientation & 0.054 & 0.030 & 1.000 & 0.030 & 0.528 & 0.040 & 0.664 & 0.040 \\
\hline
 
 \multirow{5}{*}{Farhan \etal \cite{farhan2016behavior}} & First-gen College Student & 0.246 & 0.040 & 0.646 & 0.040 & 0.370 & 0.040 & \cellcolor[HTML]{F4CCCC}*0.022 & 0.010 \\
  & Gender & 0.219 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.018 & 0.010 & 0.892 & 0.050 & 0.085 & 0.030 \\
  & Immigration Status & 0.067 & 0.020 & 0.484 & 0.030 & 0.362 & 0.030 & 0.635 & 0.050 \\
  & Race & \cellcolor[HTML]{F4CCCC}*0.042 & 0.010 & 0.707 & 0.050 & \cellcolor[HTML]{EA9999}**0.010 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.112 & 0.040 \\
  & Sexual Orientation & 0.939 & 0.050 & 0.218 & 0.020 & \cellcolor[HTML]{EA9999}**0.010 & \cellcolor[HTML]{F4CCCC}*0.020 & \cellcolor[HTML]{F4CCCC}*0.038 & 0.020 \\
\hline

 \multirow{5}{*}{Canzian \etal \cite{canzian2015trajectories}} & First-gen College Student & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.011 & \cellcolor[HTML]{F4CCCC}*0.020 & 0.214 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.023 & 0.020 \\
  & Gender & 1.000 & 0.030 & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.146 & 0.020 & \cellcolor[HTML]{F4CCCC}*0.031 & 0.030 \\
  & Immigration Status & 1.000 & 0.030 & 0.861 & 0.050 & 0.347 & 0.040 & 0.706 & 0.050 \\
  & Race & 1.000 & 0.030 & 0.104 & 0.030 & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.062 & 0.040 \\
  & Sexual Orientation & 1.000 & 0.030 & 0.414 & 0.040 & 0.440 & 0.050 & \cellcolor[HTML]{E06666}0.001 & \cellcolor[HTML]{F4CCCC}*0.010 \\
\hline
 
 \multirow{5}{*}{Wang \etal \cite{wang2018tracking}} & First-gen College Student & 0.324 & 0.040 & 1.000 & 0.030 & 0.556 & 0.050 & 0.367 & 0.030 \\
  & Gender & 0.257 & 0.030 & 1.000 & 0.030 & 0.100 & 0.020 & 0.372 & 0.040 \\
  & Immigration Status & \cellcolor[HTML]{F4CCCC}*0.019 & 0.010 & 1.000 & 0.030 & 0.103 & 0.030 & 0.920 & 0.050 \\
  & Race & 0.059 & 0.020 & 1.000 & 0.030 & 0.259 & 0.040 & 0.124 & 0.020 \\
  & Sexual Orientation & 0.618 & 0.050 & 1.000 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.029 & 0.010 & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 \\
\hline
 
 \multirow{5}{*}{Lu \etal \cite{lu2018joint}} & First-gen College Student & 0.549 & 0.030 & 0.277 & 0.050 & 0.605 & 0.040 & 0.298 & 0.030 \\
  & Gender & 0.548 & 0.020 & 0.083 & 0.020 & 0.704 & 0.050 & 0.207 & 0.020 \\
  & Immigration Status & 0.708 & 0.040 & 0.185 & 0.040 & \cellcolor[HTML]{F4CCCC}*0.040 & 0.020 & \cellcolor[HTML]{EA9999}**0.008 & \cellcolor[HTML]{F4CCCC}*0.010 \\
  & Race & 0.071 & 0.010 & 0.151 & 0.030 & 0.082 & 0.030 & 0.560 & 0.050 \\
  & Sexual Orientation & 0.929 & 0.050 & 0.082 & 0.010 & \cellcolor[HTML]{E06666}***<0.001 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.536 & 0.040 \\
\hline
 
 \multirow{5}{*}{Xu\_interpretable \etal \cite{xu2019leveraging}} & First-gen College Student & 0.996 & 0.050 & 0.068 & 0.010 & 0.290 & 0.020 & 0.524 & 0.030 \\
  & Gender & 0.969 & 0.040 & 0.143 & 0.020 & 0.790 & 0.040 & 0.063 & 0.010 \\
  & Immigration Status & 0.139 & 0.020 & 0.195 & 0.030 & 0.780 & 0.030 & 0.651 & 0.040 \\
  & Race & 0.130 & 0.010 & 0.657 & 0.040 & 0.228 & 0.010 & 0.790 & 0.050 \\
  & Sexual Orientation & 0.460 & 0.030 & 0.819 & 0.050 & 0.835 & 0.050 & 0.199 & 0.020 \\
\hline
 
 \multirow{5}{*}{Xu\_personalized \etal \cite{xu2021leveraging}} & First-gen College Student & 0.212 & 0.020 & 0.537 & 0.040 & 0.609 & 0.020 & 0.178 & 0.010 \\
  & Gender & 0.853 & 0.040 & 0.310 & 0.030 & 0.069 & 0.010 & 0.182 & 0.020 \\
  & Immigration Status & 0.941 & 0.050 & \cellcolor[HTML]{F4CCCC}*0.045 & 0.020 & 0.609 & 0.020 & 0.342 & 0.030 \\
  & Race & 0.501 & 0.030 & \cellcolor[HTML]{EA9999}**0.010 & \cellcolor[HTML]{F4CCCC}*0.010 & 0.881 & 0.050 & 0.682 & 0.040 \\
  & Sexual Orientation & 0.211 & 0.010 & 0.861 & 0.050 & 0.833 & 0.040 & 0.723 & 0.050 \\
\hline
 % \multirow{5}{*}{Chikersal \etal \cite{chikersal2021detecting}} & First-gen College Student & 0.483 & 0.020 & 0.197 & 0.020 & 0.311 & 0.030 & 0.537 & 0.050 \\
 %  & Gender & 0.725 & 0.050 & 0.654 & 0.040 & 0.420 & 0.040 & \cellcolor[HTML]{EA9999}**0.002 & \cellcolor[HTML]{F4CCCC}*0.010 \\
 %  & Immigration Status & 0.600 & 0.040 & 0.326 & 0.030 & \cellcolor[HTML]{F4CCCC}*0.022 & 0.010 & 0.455 & 0.040 \\
 %  & Race & 0.388 & 0.010 & 0.139 & 0.010 & \cellcolor[HTML]{F4CCCC}*0.030 & 0.020 & \cellcolor[HTML]{F4CCCC}*0.011 & \cellcolor[HTML]{F4CCCC}*0.020 \\
 %  & Sexual Orientation & 0.593 & 0.030 & 0.910 & 0.050 & 0.921 & 0.050 & 0.217 & 0.030 \\\hline
\end{tabular}}
\label{tab_fpr_w_t_demo}
\end{table}

==> fig_tab_alg/tab_mixed_effect_emotional_TP.tex <==
\renewcommand{\arraystretch}{0.95}
\footnotesize
\begin{longtable}{|l|l|lrrr|}
\caption{\textbf{Results of Linear Mixed Models Analysis}. This table presents the outcomes from linear mixed models, aimed at determining the significance of differences in regression models across various contexts within different engagement prediction tasks. Significance is marked *$<0.05$, **$<0.01$, ***$<0.001$. }\label{tab:case_study2_eval_results} \\
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Engagement Task}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Contextual Factors}}} & \multicolumn{4}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{Linear Mixed Model Results}} \\\cline{3-6} 
\multicolumn{1}{|c|}{}& \multicolumn{1}{c|}{}  &  & \makecell[c]{Coef.} & \makecell[c]{Std. Error} & \makecell[c]{P>|z|} \\\hline
 \multirow{25}{*}{Emotional}& 
 \multirow{3}{*}{Gender} & Intercept & 0.006  &   0.119 & 0.962 \\
 & & groups [T.Male] & -0.025  &   0.179 & 0.891  \\
 & & Group Var & 0.121  &  0.072  &   \\\cline{2-6}
 & \multirow{4}{*}{Temperature Comfort} & Intercept & -0.140 &  0.116  & 0.225  \\
 & & groups [T.No change] & 0.286 & 0.112 &  *\textbf{0.011}  \\
 & & groups [T.Warmer] & -0.117 & 0.150 & 0.436   \\
 & & Group Var & 0.112 & 0.067 & \\\cline{2-6}
 &\multirow{5}{*}{Language Room} & Intercept &  0.001  &  0.094 & 0.991   \\
 & & groups [T.Room41L] &  0.721   & 0.244 &  **\textbf{0.003}   \\
 & & groups [T.Room43L] & -0.094   &  0.184  & 0.611  \\
 & & groups [T.Room68L] & -0.351  &  0.198 & 0.076    \\
 & & Group Var & 0.057  &  0.045  &   \\\cline{2-6}
 &\multirow{4}{*}{Math Room} & Intercept & 0.194 &    0.166 & 0.242 \\
 & & groups [T.Room41M] & -0.292  &   0.215 & 0.175 \\
 & & groups [T.Room43M] &  -0.251 &    0.223 & 0.261  \\
 & & Group Var & 0.111  &  0.070 &  \\\cline{2-6}
 &\multirow{9}{*}{Courses} & Intercept & -0.285  &   0.237 & 0.228\\
 & & groups [T.English] &  0.488 &    0.241 & *\textbf{0.043} \\
 & & groups [T.Health] &  0.400  &   0.353 & 0.257  \\
 & & groups [T.Language] & 0.075 &    0.255 & 0.769  \\
 & & groups [T.Maths] &  0.274 &    0.240  & 0.253  \\
 & & groups [T.PE] &  0.485  &   0.356 & 0.173  \\
 & & groups [T.Politics] &  0.174 &    0.251  & 0.489  \\
 & & groups [T.Science] &  0.240 &     0.262 &   0.360  \\
 & & Group Var &  0.128  &  0.085 &  \\\hline
 \multirow{25}{*}{}& 
 \multirow{3}{*}{Gender} & Intercept & -0.055  &   0.121 & 0.651  \\
 & & groups [T.Male] & 0.080  &   0.182  & 0.659 \\
 & & Group Var & 0.120  &  0.070     & \\\cline{2-6}
 & \multirow{4}{*}{Temperature Comfort} & Intercept & -0.113  &   0.118 & 0.338\\
 & & groups [T.No change] &  0.181  &   0.119  & 0.130  \\
 & & groups [T.Warmer] & -0.013  &   0.160 & 0.937   \\
 & & Group Var &  0.098  &  0.054  & \\\cline{2-6}
 Cognitive &\multirow{5}{*}{Language Room} & Intercept & 0.101  &   0.114  & 0.377  \\
 & & groups [T.Room41L] & -0.492  &   0.299 &  0.100  \\
 & & groups [T.Room43L] & -0.213 &    0.219  & 0.331 \\
 & & groups [T.Room68L] &  -0.181 &    0.241  & 0.452   \\
 & & Group Var &  0.097  &  0.070   &  \\\cline{2-6}
 &\multirow{4}{*}{Math Room} & Intercept & -0.314 &    0.155 &  *\textbf{0.043}  \\
 & & groups [T.Room41M] &  0.330 &    0.201  & 0.101   \\
 & & groups [T.Room43M] & 0.500  &   0.209 & 0.017  \\
 & & Group Var & 0.086  &  0.058 &  \\\cline{2-6}
 &\multirow{9}{*}{Courses} & Intercept &  -0.376  &   0.241& 0.119   \\
 & & groups [T.English] &  0.396  &   0.246  & 0.107   \\
 & & groups [T.Health] & 0.395   &  0.360  & 0.273   \\
 & & groups [T.Language] &  -0.148  &  0.260 & 0.569 \\
 & & groups [T.Maths] &  0.530  &   0.245 &  *\textbf{0.030}  \\
 & & groups [T.PE] &  0.558  &    0.363 &   0.125  \\
 & & groups [T.Politics] &  0.212  &   0.256 &  0.407   \\
 & & groups [T.Science] & 0.634 &   0.267 & *\textbf{0.018}  \\
 & & Group Var &  0.126  &  0.073 &  \\
\hline

\multirow{25}{*}{Behavioral}& 
 \multirow{3}{*}{Gender} & Intercept & -0.055  &   0.121 & 0.651  \\
 & & groups [T.Male] & 0.080  &   0.182  & 0.659 \\
 & & Group Var & 0.120  &  0.070     & \\\cline{2-6}
 & \multirow{4}{*}{Temperature Comfort} & Intercept & -0.113  &   0.118 & 0.338\\
 & & groups [T.No change] &  0.181  &   0.119  & 0.130  \\
 & & groups [T.Warmer] & -0.013  &   0.160 & 0.937   \\
 & & Group Var &  0.098  &  0.054  & \\\cline{2-6}
 &\multirow{5}{*}{Language Room} & Intercept & 0.101  &   0.114  & 0.377  \\
 & & groups [T.Room41L] & -0.492  &   0.299 &  0.100  \\
 & & groups [T.Room43L] & -0.213 &    0.219  & 0.331 \\
 & & groups [T.Room68L] &  -0.181 &    0.241  & 0.452   \\
 & & Group Var &  0.097  &  0.070   &  \\\cline{2-6}
 &\multirow{4}{*}{Math Room} & Intercept & -0.314 &    0.155 &  *\textbf{0.043}  \\
 & & groups [T.Room41M] &  0.330 &    0.201  & 0.101   \\
 & & groups [T.Room43M] & 0.500  &   0.209 & 0.017  \\
 & & Group Var & 0.086  &  0.058 &  \\\cline{2-6}
 &\multirow{9}{*}{Courses} & Intercept &  -0.376  &   0.241& 0.119   \\
 & & groups [T.English] &  0.396  &   0.246  & 0.107   \\
 & & groups [T.Health] & 0.395   &  0.360  & 0.273   \\
 & & groups [T.Language] &  -0.148  &  0.260 & 0.569 \\
 & & groups [T.Maths] &  0.530  &   0.245 &  *\textbf{0.030}  \\
 & & groups [T.PE] &  0.558  &    0.363 &   0.125  \\
 & & groups [T.Politics] &  0.212  &   0.256 &  0.407   \\
 & & groups [T.Science] & 0.634 &   0.267 & *\textbf{0.018}  \\
 & & Group Var &  0.126  &  0.073 &  \\
\hline
\end{longtable}

\normalsize

